The Heterogeneous Capacitated $k$-Center Problem

In this paper we initiate the study of the heterogeneous capacitated $k$-center problem: given a metric space $X = (F \cup C, d)$, and a collection of capacities. The goal is to open each capacity at a unique facility location in $F$, and also to assign clients to facilities so that the number of clients assigned to any facility is at most the capacity installed; the objective is then to minimize the maximum distance between a client and its assigned facility. If all the capacities $c_i$'s are identical, the problem becomes the well-studied uniform capacitated $k$-center problem for which constant-factor approximations are known. The additional choice of determining which capacity should be installed in which location makes our problem considerably different from this problem, as well the non-uniform generalizations studied thus far in literature. In fact, one of our contributions is in relating the heterogeneous problem to special-cases of the classical Santa Claus problem. Using this connection, and by designing new algorithms for these special cases, we get the following results: (a)A quasi-polynomial time $O(\log n/\epsilon)$-approximation where every capacity is violated by $1+\varepsilon$, (b) A polynomial time $O(1)$-approximation where every capacity is violated by an $O(\log n)$ factor. We get improved results for the {\em soft-capacities} version where we can place multiple facilities in the same location.

==> full-intro.tex <==
\section{Full Version: Introduction}
The capacitated $k$-center problem is a classic optimization problem where a finite metric space $(X,d)$ needs to be partitioned into $k$ clusters so that  every  cluster has cardinality at most
some specified value $L$, and the objective is to minimize the maximum intra-cluster distance. This problem was introduced by Bar-Ilan et al~\cite{Bar-IlanKP93} and has many applications~\cite{LuptonMY98,MorganL77,Murthy1983AnAA}, including %see khuller-sussmann paper for these refs.
the {\em machine placement problem}: determine where to place a given collection of \emph{identical servers} to minimize the makespan (jobs are located in a metric space, and first need to reach the server they are assigned to before they can be processed)~\cite{PSW97}. %\mcomment{Add Venkat's References?}

The above problem is {\em homogeneous} in the sizes of the clusters, that is, it has the same cardinality constraint $L$ for each cluster. In many applications, one would ask for a \emph{heterogeneous} version of the problem where we have a different cardinality constraint for the clusters.
For instance in the network scheduling application above, suppose we had machines of differing speeds. We could possibly load higher-speed machines with more jobs than lower-speed ones. In this paper, we study  the worst-case complexity of this heterogenous version.

\begin{definition}\emph{(The \mckc Problem\footnote{Technically, we should call our problem the Heterogeneous Capacitated $k$-Supplier Problem since we can only open centers in $F$. However, we avoid making this distinction throughout this paper.}.)}
	%	\begin{itemize}[noitemsep]
	%		\item {\bf Input:} Metric space $\left(X=F\cup C, d\right)$ where $F$ are facilities and $C$ are clients.
	%		\\$~~~~~~~~~~$ Collection: $(k_1,c_1), \ldots, (k_P,c_P)$ of $P$-tuples of positive integers.
	%		\item {\bf Output:} $F_1,\ldots, F_P \subseteq F$ which are pairwise disjoint and $|F_p| \leq k_p$ for all $1\le p\leq P$. \\
	%		$~~~~~~~~~~~~$ Assignment $\phi: C\to F_1\cup F_2\cup \cdots \cup F_P$ such that for all $p$, $|\{j\in C: \phi(j)\in F_p\}|\leq c_p$.
	%		\item {\bf Objective:} Minimize $\max_{j\in C} d(j,\phi(j))$.
	%	\end{itemize}
	We are given a metric space $(X = F\cup C,d)$  where $C$ and $F$ represent the clients and facility locations.%where the set $X$ is partitioned into facilities $F$ and clients $C$.
	%Furthermore, the input contains
	We are also given a collection of {\em heterogeneous} capacities: $(k_1,c_1), (k_2,c_2),\ldots, (k_P,c_P)$ with $k_i$ copies of capacity $c_i$.
	%with $c_1 \leq c_2 \le \cdots \le c_t$,  to indicate we can open $k_p$ centers (called type $p$ centers) with capacity $c_p$ in $F$.
	The objective is to install these capacities at unique locations $F'\subseteq F$, and find an assignment $\phi:C\to F'$ of clients to these locations,
	such that for any $i\in F'$ the number of clients $j$ with $\phi(j) = i$ is at most the capacity installed at $i$, and $\max_{j\in C} d(j,\phi(j))$ is minimized.
%	The objective is to minimize
	%
	% to open these centers and assign all points of $C$ to one of these so that (a) any center of type  $p$ serves at most $c_p$ clients, and (b) the maximum distance of a client $j$ to its assigned center $i$ is minimized.
%	We use $\opt$ to denote this latter distance of the optimum solution.
	A weaker version, which we call \mckc  with soft capacities, allows multiple capacities to be installed at the same location.
\end{definition}
\noindent
Note that when all $c_p = L$ and $\sum_p k_p = k$, we get back the usual capacitated $k$-center problem.
The \mckc problem is relevant in many applications where the resources available are heterogenous. The machine placement problem is one example which has applications in network scheduling~\cite{QiuSZ15,ImM15a} and distributed databases~\cite{MorganL77,SKRN15}. Another example is that of  vehicle routing problems with  fleets of different speeds~\cite{GortzMN016}. A third relevant application may be clustering; often clusters of equal sizes are undesirable~\cite{GuhaRS01} and explicitly introducing heterogeneous constraints might lead to desirable clusters.

For the homogeneous (uniform capacities) problem, Bar-Ilan et al~\cite{Bar-IlanKP93} gave a $10$-approximation which was improved to a $6$-factor approximation by Khuller and Sussmann~\cite{KhullerS00}. One cannot get a better than $2$-approximation even for the {\em uncapacitated} $k$-center problem~\cite{HochbaumS85}. Recently, there has been focus~\cite{CyganHK12,AnBCGMS14} on the {\em non-uniform capacitated $k$-center problem}: in this problem, every facility $v\in F$ has a \emph{pre-determined} capacity $c_v$ if opened (and $0$ otherwise), and the objective is again to minimize the maximum distance of a client to its assigned open facility. We remark that the non-uniform version and our heterogeneous version seem unrelated in the sense that none is a special case of the other, and moreover, they present different sets of technical challenges to overcome.

\subsection{Main Results}

For the non-uniform problem, Cygan et al~\cite{CyganHK12} gave an $O(1)$-approximation for the problem which was improved to a $9$-approximation by An et al~\cite{AnBCGMS14}. In contrast, we show using a simple reduction that, assuming $P \neq NP$, no non-trivial approximation exists for even the soft-version of \mckc, unless we {\em violate the capacities}. This observation highlights the technical differences between our problem and the homogeneous and non-uniform versions studied thus far, and also motivates us to look at bicriteria approximation algorithms: an $(a,b)$-approximation approximates the distance objective by a factor of $a$, while violating each capacity by a factor of $b$.

%Although bicriteria approximation algorithms may be unsatisfactory, sometimes these can give unicriteria approximations for other related problems.
%We mention one application that  we alluded to above, and in fact was the starting point of this research,  which may be of independent interest.
%\begin{definition}\emph{(Machine Placement Problem for Network Scheduling.)}\label{fdef:mpp}
%	The input is a metric space $(X=F\cup C,d)$ with jobs with processing times $p_j$ at locations $C$. We are also given $P$ machines with speeds $s_1,s_2,\ldots,s_P$.
%	The goal is to find a placement of these machines on $F$ and schedule the jobs on these machines so as to minimize the makespan. The completion time of a job equals the time to reach the machine plus the processing time. In the ``soft" version of the problem, multiple machines may be placed in the same location.
%\end{definition}
%Although we do not prove it in this paper, any $(a,b)$-bicriteria approximation algorithm for (soft) \mckc problem implies an $O(a+b)$ approximation for the (soft) machine placement problem.

%The reduction in Remark~\ref{frem:cckp} does not rule out arbitrarily small violations to the capacity. Indeed the $Q||C_{min}$ problem has a PTAS~\cite{AzarE98}.
\begin{theorem}\label{fthm:1}
	Fix an $\eps > 0$. There exists an $(O(\log n/\eps), (1+\eps))$-bicriteria approximation algorithm for the \mckc problem running in time $C_\eps^{\tilde{O}(\log^3n)}$ for a constant $C_\epsilon$ depending only on $\epsilon$. For \mckc with soft capacities, there exists an $(O(\log n/\eps), (1+\eps))$-bicriteria approximation algorithm running in time $n^{O(1/\epsilon)}$.
\end{theorem}

We prove the above theorem by reducing the \mckc problems to a class of {\em max-min allocation problems} for which we design good algorithms (details appear below). Our next set of results, which also forms one of the main technical contributions of the paper, aims at reducing the logarithmic factor in the approximation to the distance. %We can give $O(1)$-approximations if the violations are allowed to be $O(1)$ in the soft-capacity case and $O(\log n)$ in the general case.
%These algorithms run in polynomial time.
\begin{theorem}\label{fthm:2}
	%For any $\eps > 0$, there exists an $\left(\tilde{O}(1/\eps), (1+\eps)\right)$-bicriteria approximation algorithm for \mckc which runs in time $n^{\tilde{O}\left(\frac{\log n}{\eps}\right)}$.
	There is a polynomial time  $(O(1),O(\log n))$-bicriteria approximation algorithm for the \mckc problem.
\end{theorem}
\begin{theorem}\label{fthm:2a}
	%For any $\eps > 0$, there exists an $\left(\tilde{O}(1/\eps), (1+\eps)\right)$-bicriteria approximation algorithm for \mckc which runs in time $n^{\tilde{O}\left(\frac{\log n}{\eps}\right)}$.
	For any $\delta>0$, there is a polynomial time  $(\tilde{O}(1/\delta),2+\delta)$-bicriteria approximation for \mckc problem with soft capacities.
\end{theorem}
\begin{corollary}
There is a polynomial time $O(\log n)$ (resp. $O(1)$) approximation for non-uniform machine placement (resp. with machine co-location allowed).
\end{corollary}
%In particular we have polynomial time $O(1)$ and $O(\log n)$ approximation algorithms for the machine placement problem of Definition~\ref{fdef:mpp}.


\subsection{Connection to Non-Uniform Max-Min Allocation Problems}
One main finding of this paper is the connection of \mckc~to the {\em non-uniform} max-min allocation (also known as Santa Claus~\cite{BansalS06}) problem. %thereby
 %underscoring the technical difficulty and difference of \mckc from  homogeneous (and also non-uniform) capacitated $k$-center. %we relate it to the classic $3$-Partitioning problem~\cite{Garey-Johnson}: in this problem
We now define these max-min allocation problems using  scheduling parlance.

\begin{definition}[$Q||C_{min}$ and \cckp]
In the\footnote{(Ab)using Graham's notation} $Q||C_{min}$ problem, one is given $m$ machines with demands $D_1,\ldots,D_m$ and $n$ jobs with capacities $c_1,\ldots,c_n$,
and the objective is to find an assignment of the jobs to machines satisfying each demand.
%We call this problem, (ab)using Graham's notation as $Q||C_{min}$.
In the {\em cardinality constrained}  non-uniform max-min allocation problem, denoted as the \cckp problem, each machine further comes with a cardinality constraint $f_i$, and a feasible solution cannot allocate more than $f_i$ jobs to machine $i$. The objective remains the same. An $\alpha$-approximate feasible solution assigns each machine $i$  total capacity at least $ D_i/\alpha$.
\end{definition}
\noindent

To show one side of the connection, we sketch how these problems arise as special cases
of \mckc, even with soft capacities.
\begin{remark}[Reduction from $Q|f_i|C_{min}$]\label{frem:cckp}
	Given an instance $\calI$ of $Q|f_i|C_{min}$, construct the instance of \mckc as follows. The capacities available to us are precisely the capacities of the jobs in $\calI$. The metric space is divided into $m$ groups $(F_1\cup C_1),\ldots,(F_m\cup C_m)$ such that the distance between nodes in any group is $0$ and across groups is $1$. Furthermore, for $1\leq i\leq m$, $|F_i| = f_i$ and $|C_i| = D_i$. Observe that the \mckc instance has a $0$-cost, capacity-preserving solution iff $\calI$ has a feasible assignment.
%	When there are soft capacities, the above reduction is from $Q||C_{min}$.
\end{remark}

Indeed, the strong NP-hardness of \cckp and $Q || C_{min}$ shows that we cannot get true approximations for \mckc, with or without soft-capacities.
As mentioned before, our main technical contribution is in showing a connection in the converse direction as well. Indeed, our algorithms in~\Cref{fthm:1,thm:2,thm:2a} use the following results we obtain for $Q|f_i|C_{min}$ and $Q||C_{min}$.

%We are not aware of non-trivial results for the \cckp problem (although, see Remark~\ref{frem:cckp-prev} below). We therefore call out the special case of the above theorem.
%This makes it rather improbable for \cckp to be APX-hard, and we leave the design of a PTAS as a challenging open problem.
\begin{theorem}\label{fthm:q}
	There is a QPTAS for the \cckp problem.
\end{theorem}


%Once again, we call out what we believe is the first polynomial time non-trivial approximation to \cckp.
\begin{theorem}\label{fthm:cckp}
	There is a poly-time $O(\log D)$ approximation algorithm for \cckp.
\end{theorem}

\begin{theorem} \label{fthm:cckp-soft}
 There is a simple $2$-approximation for $Q || C_{min}$.
 \end{theorem}

%We end the section by stating what we believe was the frontier of knowledge for the \cckp problem.
%\begin{remark}[Known algorithms for \cckp]\label{frem:cckp-prev}\emph{
	To our knowledge, \cckp has not been explicitly studied in the literature. % though the min-max version has been
	However, in a straightforward manner one can reduce \cckp to {\em non-uniform}, restricted-assignment max-min allocation problem (which we denote as $Q|restr|C_{min}$) where,  instead of the cardinality constraint dictated by $f_i$, we restrict jobs to be assigned only to a subset of the machines.\footnote{
	The reduction proceeds as follows: for every machine $i$ and job $j$, restrict $j$ to be assigned to $i$ iff $c_j \geq D_i/2f_i$. It is not hard to see that a $\rho$-approximation for the $Q|restr|C_{min}$ implies a $2\rho$-approximation for the \cckp instance.} Clearly $Q|restr|C_{min}$  is a special case of the general max-min allocation problem~\cite{ChakrabartyCK09} and therefore for any $\epsilon>0$, there are $n^{O(1/\epsilon)}$-time algorithms
achieving $O(n^\epsilon)$-approximation. We do not know of any better approximations for $Q|restr|C_{min}$. The so-called Santa Claus problem, which is the {\em uniform} version $P|restr|C_{min}$ where all demands are the same~\cite{BansalS06}, has a $O(1)$-approximations~\cite{Feige08,AsadpourFS12,PolacekS16}. However all these algorithms use the configuration LP; unfortunately for the non-uniform version $Q|restr|C_{min}$, this LP has an integrality gap of $\Omega(\sqrt{n})$ (this example is in fact the gap example of~\cite{BansalS06} for general max-min allocation -- see Appendix~\ref{fsec:app-bsig}.)%}
%\end{remark}


%%Although the violation in the capacities is large (although bounded by a constant), it already implies $O(1)$-approximations for the machine placement problem alluded to in the first paragraph.
%%This maybe of independent interest.
%\begin{theorem}\label{fthm:mpp}
%	There is a polynomial time $O(1)$-approximate algorithm for the machine placement problem.
%\end{theorem}

%The reduction from $3$-Partitioning does not rule out non-trivial approximation algorithms which violate the capacity by $(1+\epsilon)$-factor for arbitrarily small $\epsilon>0$.
%Indeed, for $3$-Partitioning, there exist algorithms~\cite{bibid} which either return No, or find a partition with $\sum_{j\in S_i} a_j \geq D(1-\eps)$. %Thus for \mckc, approximation algorithms with  arbitrarily small capacity violation is not ruled out by the above reduction.
%However, as we discuss below, many {\em cardinality constrained scheduling problems} are also special cases of the \mckc problem. There are currently no PTASes known for these problems
%and in a sense which we elaborate in Section~\ref{fsec:techs} capture the difficulty in the problem.
%Nevertheless, we are able to obtain non-trivial algorithms with $(1+\epsilon)$-capacity violation.
%
%%Our first result is an algorithm which for any $\eps>0$ returns an assignment which violates the capacities by at most $(1+\eps)$-factor and has cost at most $\tilde{O}(1/\eps)$ times $\opt$. However, it runs in quasipolynomial time.
%\begin{theorem}\label{fthm:1}
%	For any $\eps > 0$, there exists an $(O(\log n/\eps), (1+\eps))$-bicriteria approximation algorithm for the \mckc problem running in time $C_\eps^{\tilde{O}(\log^3n)}$ for a constant $C_\epsilon$ depending only on $\epsilon$.
%	%There is an $(O(1),O(1))$-bicriteria approximation algorithm for the \mckc problem.
%\end{theorem}
%%When restricted to polynomial time algorithms, we can get constant factor approximations.
%%
%%As of now we do not know whether there are $(O(1),(1+\eps))$-bicriteria approximation algorithms for the \mckc problem -- we leave this as an open problem in our paper.
%%However, for this to exist, one must first obtain PTASes for certain {\em cardinality constrained scheduling} problems looked at the literature, for which only constant factor algorithms are currently known.
%%
%%We end this section with two comments.

%We encapsulate this in the following theorem.
%
%\begin{theorem}
%	Any algorithm for \mckc violating the capacity constraints by $(1+\eps)$ would imply a PTAS for cardinality constrained max-min allocation problem on uniform speed machines.
%	%Any $(a,b)$-bicriteria approximation for \mckc implies a $b$-approximation for the cardinality constrained max-min allocation problem on uniform speed machines.
%\end{theorem}
%\noindent
%One of the main components of our algorithm for \mckc is a constant-approximation for $Q|k_i|C_{min}$. We call out this theorem as an independent interest question, and ask if there are PTAS for the same.
%\begin{theorem}\label{fthm:part2}
%	There is a $O(1)$-approximation algorithm to cardinality constrained max-min allocation problem on uniform speed machines.
%\end{theorem}
%It is natural at this point to ask the complexity of cardinality constrained max-min and min-max allocation problems on unrelated machines. For makespan minimization, Saha and Srinivasan~\cite{SS} in fact give a $2$-approximation which matches the best known algorithm without cardinality constraints. They do so by using the natural assignment LP relaxation augmented with cardinality constraints and describe a rounding algorithm.
%The max-min problem, however, is notoriously difficult~\cite{bibid} even without the cardinality constraints -- {\em describe results.} There are $O(1)$-algorithms known for the restricted-assignment max-min allocation problem~\cite{bibid} which we denote as $P|restr|C_{min}$ (also known as the Santa Claus problem); this is the same setting as $P||C_{min}$ except some jobs are disallowed on some machines.
%
%One can reduce the cardinality-constrained max-min allocation problem to the restricted assignment max-min allocation problem in the following straightforward manner. Given a guess $T$ for the optimum value, in the optimum solution machine $i$ must be allocated
%a subset of jobs $J$ such that $\sum_{j\in J} p_j \ge Ts_i/2$ {\em and} $p_j \geq Ts_i/2k_i$ for $j\in J$. Therefore, if we restrict jobs $j$ to machines $i$ only if $p_j \ge Ts_i/2k_i$, then solving this restricted assignment max-min allocation problem {\em without} cardinality constraints would give a $O(1)$-approximation. In short, the $O(1)$-approximation algorithms for the Santa Claus problem imply $O(1)$-approximation algorithms for $P|k_i|C_{min}$. Unfortunately, we do not know $O(1)$-approximation algorithms for $Q|restr|C_{min}$; all the $O(1)$-algorithms for restricted-assignment max-min problems go via classifying jobs as big or small (for all machines), and it is not clear whether the various $O(1)$-algorithms~\cite{BS, Feige, Ola, AFS}  for Santa Claus generalize to this case. We leave this as an interesting open question.
%

\subsection{Outline of Techniques} \label{fsec:overview}
As mentioned before, we obtain our results by reducing \mckc~{\em to} the \cckp problem (complementing the {\em from} reduction  discussed in Remark~\ref{frem:cckp}).
We provide two reductions -- the first incurs logarithmic approximation to the cost but uses black-box algorithms for \cckp, the second incurs $O(1)$-approximation to the cost but uses ``LP-based'' algorithms for \cckp.
%Both these reductions proceed via {\em decomposing} the given \mckc instance. %\smallskip

\medskip \noindent {\bf Warm-up: Weak Decompostion.}
Given a \mckc instance, suppose we \emph{guess} the optimal objective value, which we can assume to be $1$ after scaling. Then, we construct a graph connecting client $j$ with facility location $i$ iff $d(i,j) \leq 1$.
Then, starting at an arbitrary client and using a simple region-growing technique (like those used for the graph cut problems~\cite{LeightonR99,GargVY96}), we can find a set of clients $J_1$ of along with their neighboring facility locations $T_1 = \Gamma(J_1)$\footnote{For $S \subseteq C \cup F$, $\Gamma(S)$ denotes the neighboring vertices  of $S$.}, such that: (a) the diameter of $J_1$ is $O(\log n/\epsilon)$, and (b) the additional clients in the boundary $|\Gamma(T_1) \setminus J_1|$ is at most $\epsilon |J_1|$. Now, we simply \emph{delete} these boundary clients and charge them to $J_1$, incurring a capacity violation of $(1+\epsilon)$. Moreover, note that in an optimal solution, \emph{all} the clients in $J_1$ \emph{must be} assigned to facilities opened in $T_1$. Using this fact, we define our first demand in the \cckp instance by $D_1 = |J_1|$ and $f_1 = |T_1|$. Repeating this process, we get a collection of $\{(J_i,T_i)\}$ which naturally defines our \cckp instance. It is easy to show that any $\alpha$-approximation to the \cckp instance then implies an $(O(\log n/\epsilon),  \alpha(1+\epsilon))$-bicriteria algorithm for \mckc.

\iffalse
The weaker decomposition theorem (Theorem~\ref{fthm:weakdecomp}) states that we can delete a subset $\Cd$ of clients and partition the residual instance into portions we call {\em complete neighborhood sets} (Definition~\ref{fdef:comp-nbr}) of $O(\log n/\epsilon)$ diameter.
These sets consists of subsets of facilities $T_i$ and clients $J_i$ such that the optimal solution \emph{must} assign clients in $J_i$ to facilities in $T_i$. This collection of complete-neighborhood sets then naturally leads to a \cckp instance (Remark~\ref{frem:red})
whose solutions translate to \mckc solutions with $O(\log n/\epsilon)$ hit on the cost. Furthermore, the deleted clients $\Cd$ can be charged to clients in $C\setminus \Cd$ such that the capacity of facilities only increase by an $\epsilon$-factor.
We use the {\em region growing technique} which have been used for cut problems~\cite{LeightonR99,GargVY96} to find the set $\Cd$; we keep on growing balls till the total external demand is at most $\epsilon$ times the internal demand.
$O(\log n/\eps)$-radius balls suffice. %\smallskip
\fi

\medskip \noindent {\bf LP-Based Strong Decompostion.} %It is not a-priori clear how to modify the above technique to obtain better factors for the distance objective.
To get $O(1)$-approximations, we resort to linear programming relaxations. Indeed, one can write the natural LP relaxation \eqref{feq:lp1}-\eqref{feq:lp6} described in Section~\ref{fsec:prelims} -- the relaxation has $y_{ip}$ variables which denote opening a
facility with capacity $c_p$ at $i$.
Armed with a feasible solution to the LP, we prove a \emph{stronger decomposition theorem} (Theorem~\ref{fthm:decomp}): we show that we can delete a set of clients $\Cd$ which can be charged to the remaining ones, and then partition the set of clients and facilities into {\em two} classes.
One class $\calT$  is the so-called \emph{complete neighborhood sets} of the form $\{(J_i, T_i)\}$ with $\Gamma(J_i) \subseteq T_i$ as described above. The other class $\calS$  is of, what we call, {\em roundable} sets (Definition~\ref{fdef:rnding-mkc}). Roundable sets have ``enough'' $y$-mass such that installing as many  capacities as prescribed by the LP (rounded down to the nearest integer) supports the total demand incident on the set (with a $(1+\epsilon)$-factor capacity violation). Moreover, the diameter of any of these sets constructed is $\tilde{O}(1/\epsilon)$.

\medskip \noindent {\bf Technical Roadblock.}
It may seem that the above decomposition theorem implies a reduction to the \cckp problem -- the class $\calT$ defines a \cckp instance and we can use black-box algorithms, while the roundable sets in $\calS$ are taken care of almost by definition. The nub of the problem lies in the {\em supply} of capacities to each of these classes.  Indeed, the \cckp instance formed from $\calT$ must have a solution if the \mckc problem is feasible, {\em but only if all the $k_p$ copies of capacity $c_p$ are available to it.} However, we have already used up some of these copies to take care of the $\calS$ sets, and what we actually have available for $\calT$ is what the {\em LP prescribes.} In fact, this natural LP relaxation (and the natural LP for \cckp) have arbitrarily bad integrality gaps, even for bicriteria algorithms.%, that is, although the LP is feasible, any assignment will violate capacities to $\Omega(n)$ factors.% \smallskip

\medskip \noindent {\bf The Supply Polyhedra.} We circumvent this issue in the following manner: the above method would be fine if the supply of facility capacities prescribed by the LP to the complete-neighborhood sets in $\calT$ can approximately satisfy the demands in the corresponding \cckp instance. This motivates us to define {\em supply polyhedra} for \cckp. Informally, the supply polyhedron (Definition~\ref{fdef:supp-poly}) of a \cckp instance is supposed to capture all the vectors $(s_1,\ldots,s_n)$ such that $s_j$ copies of capacity $c_j$ can approximately satisfy the demands of all the machines. Conversely, any vector in this polyhedron should also be a feasible (or approximately feasible) supply vector for this instance.

 If such an object $\calP$ existed, then we could strengthen our natural LP relaxation as follows. For {\em every} collection $\calT$ of complete-neighborhood sets, we add a constraint (described as \eqref{feq:lp7}) stating that the fractional capacity allocated to the facilities in $\calT$ should
 lie in the supply polyhedron of the corresponding \cckp instance. Note that this LP has exponentially many constraints, and it is not clear how to solve it. However, we can use the ``round-and-cut'' framework (of inferring a separating hyperplane using our rounding algorithm, and then using the ellipsoid algorithm overall) exploited earlier in many papers~\cite{CarrFLP00,ChakrabartyCKK11,AnSS14,DemirciL16,Li15,Li16}.
 %Starting with a solution $(x,y)$, we use the strong decomposition theorem to obtain the set $\calT$ and check if the restriction of $y$ to the facilities in $\calT$ lies in the supply polyhedron of the corresponding \cckp instance. If yes, then we are done.
 %If no, then we have obtained a separating hyperplance for the super-large LP\eqref{feq:lp1}-\eqref{feq:lp7}, and we can run the ellipsoid algorithm.
 Using this decomposition, in~\Cref{fthm:reduction}, we effectively reduce \mckc to the task of designing good supply polyhedra for \cckp.

\medskip \noindent {\bf Supply Polyhedron for \cckp and $Q||C_{min}$.}
Do good supply polyhedra exist for \cckp or even the simpler $Q||C_{min} $ problem?
On the positive side, we show (Theorem~\ref{ffthm:asslp}) that the natural assignment LP is a $2$-approximate supply polyhedron for $Q||C_{min}$. For \cckp we describe a supply polyhedron based on the {\em configuration LP} and prove that it is $O(\log D)$-approximate (Theorem~\ref{fthm:conflp}) where $D$ is the ratio of maximum and minimum demand. This along with our strong decomposition proves Theorem~\ref{fthm:2}. This also implies a {\em polynomial time} $O(\log D)$-approximation algorithm for the \cckp problem, improving considerably over the best known guarantees implied by the current santa-claus algorithms. %Our algorithm (described in Section~\ref{fsec:conflp}) proceeds by massaging a given LP solution till it yields.
%\comment{Do we want to add a line on how we get these results}
We complement this by showing (Theorem~\ref{ffthm:conf-ig}) that the integrality gap of the configuration LP is $\Omega(\log D/\log\log D)$, using which we also show a \emph{lower-bound} on the approximation factor possible using supply polyhedra: any supply polyhedra for \cckp must violate the demands by $\Omega(\log D/\log \log D)$. This shows that our approach inherently needs to violate capacities by this factor.

%On the other hand, using fairly standard tricks of enumeration and rounding, we can provide a QPTAS for \cckp (Theorem~\ref{fthm:q}). We leave the complexity of \cckp as an interesting open question.

%\paragraph{Supply Polyhedra.}




%We start by writing the natural assignment LP relaxation for the problem. As is usual, we guess $\opt$ and scale everything such that $\opt = 1$.
%We have opening  variables $y_{ip}$ for every $i\in F,p\in [P]$ indicating whether we open a facility with capacity $c_p$ at location $i$.
%We have connection variables $x_{ijp}$ indicating the fraction to which client $j\in C$ connects to a facility at location $i$ where a type $p$ facility has been opened.
%We force $x_{ijp} = 0$ for all $d(i,j) > 1$.
%If $\opt = 1$, there is a feasible $(x,y)$ solution to the following system of inequalities.\smallskip

%\begin{minipage}{0.45\textwidth}
%	\begin{alignat}{4}
%		& \quad \forall j\in C,   &&\quad  \textstyle \sum_{i\in F} \sum_{p\in [P]}  x_{ijp} \geq 1 \label{feq:lp1} \\
%		& \quad \forall i\in F,p\in [P] ,  &&\quad  \textstyle \sum_{j\in C}  x_{ijp} \leq c_py_{ip} \label{feq:lp2} \\
%		& \quad \forall p\in [P], && \quad \textstyle \sum_{q \geq p} y_{iq}   \leq \sum_{q\geq p} k_q \label{feq:lp3}
%	\end{alignat}
%\end{minipage}
%~\vline~
%\begin{minipage}{0.45\textwidth}
%	\begin{alignat}{4}
%		& \quad \forall i\in F, j\in C,p\in [P],  && \quad x_{ijp} \leq y_{ip}\label{feq:lp4}   \\
%		& \quad \forall i\in F, && \quad \textstyle\sum_{p\in [P]} y_{ip} \leq 1 \label{feq:lp5}  \\
%		& \quad \forall i\in F,j\in C,p\in [P], && \quad x_{ijp},y_{ip} \geq 0\label{feq:lp6}
%	\end{alignat}
%\end{minipage}
%\smallskip

%For technical reasons, we have written \eqref{feq:lp3} as a constraint on the prefix-sums rather than individual capacities. However, a feasible integral solution satisfying \eqref{feq:lp3} can easily be converted to a feasible solution satisfying individual capacities.

%\paragraph{Integrality Gap.}
%The above LP has bad integrality gap even when we allow arbitrary violation of capacities.
%Consider the following instance. The metric space $X$ is partitioned into $(F_1\cup C_1) \cup \cdots \cup (F_K\cup C_K)$, with $|F_k| = 2$ and $|C_k| = K$ for all $1\le k\le K$.
%The distance between any two points in $F_i\cup C_i$ is $1$ for all $i$, while all other distances are $\infty$. The capacities available are $k_1 = K$ facilities with capacity $c_1 = 1$ and
%$k_2= K-1$ facilities with capacity $c_2 = K$. It is easy to see that integrally any solution would violate capacities by a factor of $K/2$.
%%It is easy to see that the above instance is not feasible with $OPT=1$: indeed, there is at least one client location where the optimal solution does not place a facility of capacity $H$ in its neighborhood, and it is not possible to serve the demand of this client using only capacity $1$ facilities, as there are only two locations where we can place facilities in its neighborhood.
%On the other hand, there is a feasible solution for the above LP relaxation: for $F_k = \{a_k,b_k\}$, we set $y_{a_k2} = 1-1/K$ and $y_{b_k1} = 1$, and for all $j\in C_k$, we set $x_{a_kj2} = 1-1/K$ and $x_{b_kj1} = 1/K$.
%%
%%
%%fractionally assign $1-\frac1H$ units of capacity-$H$ facility and $1$ unit of capacity-$1$ facility in the neighborhood around each client. It is easy to see that there is a feasible fractional assignment of this kind which means that the LP suffers from an unbounded (w.r.t the guessed objective function value) integrality gap.
%
%
%\paragraph{Decomposition Theorem.}
%The integrality gap suggests we need to strengthen our LP, and we will indeed do so. However, the above LP suffices to tease out the instance into parts that are indeed ``well roundable'' and problematic parts which look like the example above.
%To make this precise, let us introduce two definitions.
%\begin{asparaitem}
%	\item A subset of facilities $S$ is said to be {\em $(a,b)$-roundable wrt a feasible solution $(x,y)$} to \eqref{feq:lp1}-\eqref{feq:lp6} if its diameter is at most $a$ and there is a rounding $Y_{ip}\in \{0,1\}$ for all $i\in S,p\in [P]$
%	such that the rounded solution satisfies cardinality constraints, and  has enough capacity to satisfy $1/b$th of  the {\em fractional} demand incident on $S$. In other words, if we install $b\cdot c_p$ capacity at the location where $Y_{ip} = 1$, then it can satisfy the fractional demand incident on $S$.
%	%That is, if we increase the capacities by $b$ times, there is an integral rounding of facilities in $S$.
%	\item
%	A subset $S$ of facilities is called a {\em complete neighborhood} if there exists some clients $J\subseteq C$ such that $S$ contains all the facilities in distance one to clients in $J$.  That is, for all $j\in J$, the only facilities $i$ with $x_{ijp} > 0$ must lie in $S$.
%	Note that in the integrality gap example above, the $F_k$'s are all complete neighborhoods due to the client set $C_k$'s. Also note that these complete neighborhood sets are also encountered in the reductions from $3$-Partition and the cardinality constrained scheduling problems.
%\end{asparaitem}
%
%Note that if our instance can be partitioned into roundable sets then we would be done. If our instance consists of only complete neighborhood sets, then we could hope to use techniques developed for scheduling algorithms. However, a priori, the instances are a mixture of both.
%Our main technical hammer is the decomposition theorem (Theorem~\ref{fthm:decomp}) which says that given feasible solution $(x,y)$ to \eqref{feq:lp1}-\eqref{feq:lp6}, in polynomial time we can decompose the instance $(F\cup C,d)$ into two collections $\calS$ and $\calT$ where
%every set $S$ in $\calS$ is a $(\tilde{O}(1/\eps),(1+\eps))$-roundable set, and every set $T\in \calT$ is a complete neighborhood set of diameter $\leq 4$. This tells us that the core difficulty that the above LP faces are indeed complete neighborhood sets of small diameter, and shows us how to strengthen our LP relaxation. {\bf Maybe add a few lines on how we obtain -- connections to region growing algorithms.} \medskip
%
%\noindent
%Next we describe two ways to strengthen the LP. One leads to a polynomial time algorjthm but gives $O(1)$-factor violation of the capacities, the other leads to a quasipolynomial time $(1+\eps)$-factor violation in the capacities. Both LPs, put extra constraints on the vector
%of $y_{ip}$'s. Interestingly, both LPs have exponentially number of variables and constraints we do not know if either LP is polynomial or quasipolynomial time solvable. Rather, we use the ``round-and-cut'' strategy~\cite{bunch fof citations} where the constraints+auxiliary variables are added
%in phases {\em only if} a rounding algorithm fails. This technique has led to many new algorithms in the recent past, and ours adds to this canon of growing work.
%
%\paragraph{LP strengthening.} One useful idea that has helped for scheduling problems~\cite{bibid} is to look at {\em configuration LP}. For our problem, we add the following constraint. For a subset of clients $J\subseteq C$ let $\Gamma(J)\subseteq F$
%be the facilities at distance $1$. Since $J$ can only be assigned to clients in $\Gamma(J)$, there must be enough capacity installed on $\Gamma(J)$ -- in particular, the multiset/configuration  $S$ of capacities must be of cardinality $\le |\Gamma(J)|$ and total capacity $\geq |J|$.
%We strengthen our LP~\eqref{feq:lp1}-\eqref{feq:lp6} by adding that for every $J\subseteq C$, the $y_{ip}$ vector must {\em dominate} a feasible configuration LP solution for the complete neighborhood $(\Gamma(J),J)$.
%
%As mentioned above, this huge LP is perhaps not solvable in polynomial time. Instead we add these constraints iteratively. In every phase, given a feasible $(x,y)$ to \eqref{feq:lp1}-\eqref{feq:lp6}, we apply our decomposition theorem and obtain the complete neighborhood sets and add the strengthened constraints for these sets. The analysis of the ellipsoid algorithm implies in polynomially many phases we will reach a solution $(x,y)$ where the $y$'s satisfy the configuration LP constraints for all the complete neighborhood sets.
%Our final contribution is an $O(1)$-rounding of the configuration LP. {\bf deepc: maybe expand on this as well.}
%
%



\subsection{Related Work}\label{fsec:related}
Capacitated Location problems have a rich literature although most of the work has focused on versions where each facility arrives with a predetermined capacity and the decision process is to whether open a facility or not.
We have already mentioned the state of the art for capacitated $k$-center problems.
For the capacitated facility location problem a $5$-approximation is known via local search~\cite{BansalGG12}, while more recently an $O(1)$-approximate {\em LP-based} algorithm was proposed~\cite{AnSS14}.
All these are true approximation algorithms in that they do not violate capacities. It is an outstanding open problem to obtain true approximations for the capacitated $k$-median problem.
The best known algorithm is  the recent work of  Demirci and Li~\cite{DemirciL16} who for any $\epsilon>0$ give a $\poly(1/\epsilon)$-approximate algorithm violating the capacities by $(1+\epsilon)$-factor.
The technique of this algorithm and its precursors~\cite{AnSS14,Li15,Li16}  are similar to ours in that they follow the round-and-cut strategy to exploit exponential sized linear programming relaxations.\smallskip

The \cckp problem is a cardinality constrained max-min allocation problem. There has been some work in the scheduling literature on cardinality-constrained min-max problem.
When all the machines are identical, the problem is called the $k_i$-partitioning problem~\cite{BabelKK98}.
When the number of machines is a constant, Woeginger~\cite{Woe05} gives a FPTAS for the problem, and the best known result is a $1.5$-approximation due to Kellerer and Kotov~\cite{KellererK11}.
To our knowledge, the related speeds case has not been looked at. When the machines are unrelated,  Saha and Srinivasan~\cite{SahaS10} showed a $2$-approximation; in fact this follows from the Shmoys-Tardos rounding of the assignment LP~\cite{ShmoysT93}.\smallskip

As we have discussed above, the \mckc problem behaves rather differently than the usual homogeneous capacitated $k$-center problem. This distinction in complexity when we have heterogeneity  in resource is a curious phenomenon which deserves more attention.
A previous work~\cite{ChakrabartyGK16} of the first two authors (with P.~Goyal) looked at the (uncapacitated) $k$-center problem where the heterogeneity was in the radius of the balls covering the metric space.
As in our work, even for that problem one needs to resort to bicriteria algorithms where the two criteria are cost and {\em number} of centers opened. That paper gives an $\left(O(1),O(1)\right)$-approximation algorithm.
In contrast, we do not wish to violate the number of capacities available at all (in fact, the problem is considerably easier if we are allowed to do so -- we do not expand on this any further).







==> full-preliminaries.tex <==
%\newpage
\section{Technical Preliminaries}\label{fsec:prelims}
Given an \mckc instance, we start by guessing $\opt$. We either prove $\opt$ is infeasible, or find an $(a,b)$-approximate allocation of clients to facilities.
	We define the bipartite graph $G = (F\cup C,E)$ where $(i,j)\in E$ iff $d(i,j) \leq \opt$. If $\opt$ is feasible, then the following assignment LP\eqref{feq:lp1}-\eqref{feq:lp6}
	must have a feasible solution.
In this LP, we  have opening  variables $y_{ip}$ for every $i\in F,p\in [P]$ indicating whether we open a facility with capacity $c_p$ at location $i$. Recall that the capacities available to us are $c_1, c_2, \ldots, c_P$ -- a facility with
capacity $c_p$ installed on it will be referred to as a {\em type $p$ facility.}
	We have connection variables $x_{ijp}$ indicating the fraction to which client $j\in C$ connects to a facility at location $i$ where a type $p$ facility has been opened.
	We force $x_{ijp} = 0$ for all pairs $i,j$ and type $p$ such that  $d(i,j) > \opt$.
	
		
		\begin{minipage}{0.49\textwidth}
			\begin{alignat}{3}
				& \forall j\in C,   &\textstyle \sum_{i\in F} \sum_{p\in [P]}  x_{ijp} \geq 1 \label{feq:lp1} \tag{\small{L1}}  \\
				& \forall i\in F,p\in [P] ,  &\textstyle \sum_{j\in C}  x_{ijp} \leq c_py_{ip} \label{feq:lp2} \tag{\small{L2}} \\
				& \forall p\in [P], & \textstyle \sum_{i\in F} y_{iq}   \leq k_p \label{feq:lp3}  \tag{\small{L3}}
			\end{alignat}
		\end{minipage}
		~\vline~
		\begin{minipage}{0.49\textwidth}
			\begin{alignat}{3}
				& \forall i\in F, j\in C,p\in [P],  &  x_{ijp} \leq y_{ip}\label{feq:lp4}   \tag{\small{L4}} \\
				& \forall i\in F, &  \textstyle\sum_{p\in [P]} y_{ip} \leq 1 \label{feq:lp5}  \tag{\small{L5}} \\
				& \forall i\in F,j\in C,p\in [P], &  x_{ijp},y_{ip} \geq 0\label{feq:lp6}\tag{\small{L6}}
			\end{alignat}
		\end{minipage}
\smallskip

\noindent		
We say a solution $(x,y)$ is $(a,b)$-feasible if it satisfies \eqref{feq:lp1}, \eqref{feq:lp3}-\eqref{feq:lp6}, and \eqref{feq:lp2} with the RHS replaced by $bc_py^\mathsf{int}_{ip}$, and $x_{ijp} > 0$ only if $d(i,j) \leq a\cdot \opt$,
We desire to find an integral solution $(x^\mathsf{int},y^\mathsf{int})$ which is $(a,b)$-feasible.
The following lemma shows that it suffices just to round the $y$-variables.
\begin{claim}
Given an $(a,b)$-feasible solution $(x,\y)$ where $\y_{ip}\in \{0,1\}$,
we can get  an $(a,b)$-approximate solution to the \mckc problem.
\end{claim}
\begin{proof}
Consider a bipartite graph with client nodes $C$ on one side, and nodes of the form $(i,p)$ with $\y_{ip} = 1$ on the other. The node $(i,p)$ has capacity $bc_p$.
Since $(x,\y)$ satisfies the conditions of the lemma, there is a fractional matching in this graph so that each client $j$  is fractionally matched to an $(i,p)$ so that $d(i,j)\leq a\cdot \opt$,
and the total fractional load on $(i,p)$ is $\leq bc_p$. The theory of matching tells us that there is an {\em integral} assignment of clients $j$ to nodes $(i,p)$ such that $d(i,j)\leq a\cdot\opt$
and the number of nodes matched to $(i,p)$ is $\leq \ceil{bc_p}$. Therefore opening a capacity $c_p$ facility at $i$ for all $(i,p)$ with $\y_{ip} = 1$ gives an $(a,b)$-approximate solution to \mckc.
\end{proof}
\noindent
Henceforth, we focus on rounding the $y$-values. To this end, we make the following useful definition.
\begin{definition}[Roundable Sets]\label{fdef:rnding-mkc}
	A set of facilities $S\subseteq F$ is said to be $(a,b)$-roundable w.r.t $(x,y)$ if
	\begin{itemize}[noitemsep]
		\item[(a)] $\diam_G(S) \leq a$
		\item[(b)] there exists a rounding $\y_{ip} \in \{0,1\}$ for all $i \in S, p\in [P]$ such that
		\begin{enumerate}
			\item $\sum_{q \geq p} \sum_{i\in S} \y_{iq} ~\leq~ \floor{\sum_{q \geq p}\sum_{i\in S} y_{iq}}$ for all $p$, and
			\item $\sum_{j\in C} d_j \sum_{i\in S,p\in [P]} x_{ijp} \leq b\cdot \sum_{i\in S} \sum_{p\in [P]} c_p \y_{ip}$
		\end{enumerate}
	\end{itemize}
\end{definition}
\noindent
If $(x,y)$ were feasible, then for any $(a,b)$-roundable set, we can integrally open facilities to satisfy all the demand that was fractionally assigned to it taking a hit of $a$ in the cost and a factor of $b$ in the capacities. Furthermore, the number of open facilities is at most what the LP prescribes. Therefore, if we would be able to decompose the instance into roundable sets, we would be done.
Unfortunately, that is not possible, and in fact the above LP has a large integrality gap even when we allow arbitrary violation of capacities.

\begin{remark}[Integrality Gap for \mckc] \label{frem:ig}
Consider the following instance. The metric space $X$ is partitioned into $(F_1\cup C_1) \cup \cdots \cup (F_K\cup C_K)$, with $|F_k| = 2$ and $|C_k| = K$ for all $1\le k\le K$.
The distance between any two points in $F_i\cup C_i$ is $1$ for all $i$, while all other distances are $\infty$. The capacities available are $k_1 = K$ facilities with capacity $c_1 = 1$ and
$k_2= K-1$ facilities with capacity $c_2 = K$. It is easy to see that integrally any solution would violate capacities by a factor of $K/2$.
%It is easy to see that the above instance is not feasible with $OPT=1$: indeed, there is at least one client location where the optimal solution does not place a facility of capacity $H$ in its neighborhood, and it is not possible to serve the demand of this client using only capacity $1$ facilities, as there are only two locations where we can place facilities in its neighborhood.
On the other hand, there is a feasible solution for the above LP relaxation: for $F_k = \{a_k,b_k\}$, we set $y_{a_k2} = 1-1/K$ and $y_{b_k1} = 1$, and for all $j\in C_k$, we set $x_{a_kj2} = 1-1/K$ and $x_{b_kj1} = 1/K$.


 For the version with soft capacities, we do not have the constraint \eqref{feq:lp5} and the above integrality gap doesn't hold since we can install capacity $K$ facilities on $K-1$ of the sets $F_k$'s, $1\leq k\leq K-1$, and $K$ copies of the capacity $1$ facilities at $F_K$. Note that although $|F_K| = 2$, we have opened $K$ capacities.
\end{remark}

In particular, note that for the $(x,y)$ solution in the integrality gap example above there are no roundable sets. This motivates the definition of the second kind of sets.

\begin{definition}[Complete Neighborhood Sets] \label{fdef:comp-nbr}
	A subset $T\subseteq F$ of facilities is called a {\em complete neighborhood} if there exists a client-set $J\subseteq C$ such that $\Gamma(J) \subseteq T$.
	In this case $J$ is said to be {\em responsible} for $T$. Additionally, a complete neighborhood $T$ is said to be an $\alpha$-complete neighborhood if $\diam(T) \leq \alpha$.
\end{definition}
\begin{remark}[Complete Neighborhood Sets to \cckp]\label{frem:red}
	\emph{
If we find a complete neighborhood $T$ of facilities with say a set $J$ of clients responsible for it, then we know that the optimal solution must satisfy all the demand in $J$ by suitably opening facilities of sufficient capacity in $S$. Given a collection $\calT = (T_1,\ldots,T_m)$ of disjoint $\alpha$-complete neighborhood sets with $J_i$ repsonsible for $T_i$, we can define an instance $\calI$ of the \cckp problem with $m$ machines with demands $D_i = |T_i|$ and cardinality constraint $f_i = |T_i|$, and $P$ jobs of capacities $c_1,\ldots,c_P$. The facilities opened by the $\opt $ solution corresponds to a valid solution for $\calI$; furthermore, any $\beta$-approximate solution for $\calI$ corresponds to a $(\alpha,\beta)$-approximate solution for the \mckc problem restricted to clients in $\cup_{\ell} J_\ell$. Finally note that for \mckc with soft-capacities, $\calI$ is an instance of the $Q||C_{min}$ problem.
}

\emph{
Note that the above integrality gap  example is essentially a \cckp instance with $K$ machines of demand $K$ each having cardinality constraint $2$, and there are $K$ jobs of capacity $1$ and $K-1$ jobs with capacity $K$. This shows the assignment LP has bad integrality gap for the \cckp problem (but not for $Q||C_{min}$).}
\end{remark}

Our final definition is that of $(\tau,\rho)$-{\em deletable clients} who can be removed from the instance since they can be ``$\rho$-charged'' to the remaining clients no further than $\tau$-away.
\begin{definition}[Deletable Clients]\label{fdef:deletable}
	A subset $\Cd\subseteq C$ of clients is $\rho$-deletable if there exists a mapping $\phi_{j,j'}\in [0,1]$ for $j\in \Cd$ and $j'\in C\setminus \Cd$ satisfying (a) $\sum_{j'\in C\setminus \Cd} \phi_{j,j'} = 1$ for all $j\in \Cd$, and(b) $\sum_{j\in \Cd} \phi_{j,j'} \leq \rho$ for all $j'\in C\setminus \Cd$. Furthermore, $\phi_{j,j'} > 0$ only if $d(j,j') \leq \tau\cdot\opt$.
\end{definition}
 The following claim shows we can remove $\Cd$ from consideration.
\begin{claim}\label{fclm:prelim3}
	Let $\Cd$ be a $(\rho,\tau)$-deletable set.
	Given an $(a,b)$-approximate feasible solution $(x',\y)$ where $x'_{ijp}$ is defined only for $j\in C\setminus \Cd$, we can extend $x'$ to a general $(x,\y)$ solution
	which is $(a+\tau, b(1+\rho))$-approximate feasible.
\end{claim}
\begin{proof}
For any $j\in \Cd$, define $x_{ijp} = \sum_{j'\in C\setminus \Cd} x_{ij'p}\phi_{j,j'}$.
We get for all $j\in \Cd$,
$\textstyle \sum_{i\in F} \sum_{p\in [P]} x_{ijp} = \sum_{i,p} \sum_{j'\in C\setminus \Cd} x_{ij'p}\phi_{j,j'} = \sum_{j'\in C\setminus \Cd} \phi_{j,j'} \left(\sum_{i,p} x_{ij'p}\right) \geq \sum_{j'\in C\setminus \Cd} \phi_{j,j'} = 1$,
and for all $i\in F,p\in [P]$,
$\textstyle \sum_{j\in \Cd}  x_{ijp} = \sum_{j\in \Cd} \sum_{j'\in C\setminus \Cd} x_{ij'p}\phi_{j,j'} = \sum_{j'\in C\setminus \Cd} x_{ij'p}\left( \sum_{j\in \Cd} \phi_{j,j'}\right)  \leq \rho \sum_{j'\in C\setminus \Cd} x_{ijp} \leq b\rho c_p$. Therefore, in all we have $\sum_{j\in C} x_{ijp} \leq bc_p(1+\rho)$.
\end{proof}


% described in Idea 1.







==> preliminaries.tex <==
%\newpage
\section{Preliminaries}\label{sec:prelims}
Given a \mckc instance, we start by guessing $\opt$. We either prove $\opt$ is infeasible, or find an $(a,b)$-approximate allocation of clients to facilities.
	We define the bipartite graph $G = (F\cup C,E)$ where $(i,j)\in E$ iff $d(i,j) \leq \opt$. If $\opt$ is feasible, then the following assignment LP\eqref{eq:lp1}-\eqref{eq:lp6}
	must have a feasible solution.
In this LP, we  have opening  variables $y_{ip}$ for every $i\in F,p\in [P]$ indicating whether we open a facility with capacity $c_p$ at location $i$. Recall that the capacities available to us are $c_1, c_2, \ldots, c_P$ -- a facility with
capacity $c_p$ installed on it will be referred to as a {\em type $p$ facility.}
	We have connection variables $x_{ijp}$ indicating the fraction to which client $j\in C$ connects to a facility at location $i$ where a type $p$ facility has been opened.
	We force $x_{ijp} = 0$ for all pairs $i,j$ and type $p$ such that  $d(i,j) > \opt$.
	
		
		\begin{minipage}{0.49\textwidth}
			\begin{alignat*}{2}
				 \forall j\in C,   &\textstyle \sum_{i\in F} \sum_{p\in [P]}  x_{ijp} \geq 1 \label{eq:lp1} \tag{\small{L1}}  \\
				 \forall i\in F,p\in [P] ,  &\textstyle \sum_{j\in C}  x_{ijp} \leq c_py_{ip} \label{eq:lp2} \tag{\small{L2}} \\
				 \forall p\in [P], & \textstyle \sum_{i\in F} y_{iq}   \leq k_p \label{eq:lp3}  \tag{\small{L3}}
			\end{alignat*}
		\end{minipage}
		~\vline~
		\begin{minipage}{0.49\textwidth}
			\begin{alignat*}{3}
				&\forall i\in F, j\in C,p\in [P],  & x_{ijp} \leq y_{ip}\label{eq:lp4}   \tag{\small{L4}} \\
				& \forall i\in F, & \textstyle\sum_{p\in [P]} y_{ip} \leq 1 \label{eq:lp5}  \tag{\small{L5}} \\
				& \forall i\in F,j\in C,p\in [P], & x_{ijp},y_{ip} \geq 0\label{eq:lp6}\tag{\small{L6}}
			\end{alignat*}
		\end{minipage}
\smallskip

\noindent		
We say a solution $(x,y)$ is $(a,b)$-feasible if it satisfies \eqref{eq:lp1}, \eqref{eq:lp3}-\eqref{eq:lp6}, and \eqref{eq:lp2} with the RHS replaced by $bc_py^\mathsf{int}_{ip}$, and $x_{ijp} > 0$ only if $d(i,j) \leq a\cdot \opt$.
%We desire to find an integral solution $(x^\mathsf{int},y^\mathsf{int})$ which is $(a,b)$-feasible.
%The following claim shows that it suffices just to round the $y$-variables.
\begin{claim}
Given an $(a,b)$-feasible solution $(x,\y)$ where $\y_{ip}\in \{0,1\}$,
we can get  an $(a,b)$-approximate solution to the \mckc problem.
\end{claim}
\iffalse
\begin{proof}
Consider a bipartite graph with client nodes $C$ on one side, and nodes of the form $(i,p)$ with $\y_{ip} = 1$ on the other. The node $(i,p)$ has capacity $bc_p$.
Since $(x,\y)$ satisfies the conditions of the lemma, there is a fractional matching in this graph so that each client $j$  is fractionally matched to an $(i,p)$ so that $d(i,j)\leq a\cdot \opt$,
and the total fractional load on $(i,p)$ is $\leq bc_p$. The theory of matching tells us that there is an {\em integral} assignment of clients $j$ to nodes $(i,p)$ such that $d(i,j)\leq a\cdot\opt$
and the number of nodes matched to $(i,p)$ is $\leq \ceil{bc_p}$. Therefore opening a capacity $c_p$ facility at $i$ for all $(i,p)$ with $\y_{ip} = 1$ gives an $(a,b)$-approximate solution to \mckc.
\end{proof}
\fi

We remark that as is, the LP has an unbounded integrality gap for \mckc, and indeed, the gap instances also happen to be of the \cckp variety. So we strengthen it by adding some additional constraints which we explain later. However, since our strong decomposition theorem merely uses these $y_{ip}$ and $x_{ijp}$ values, we present that first. %Henceforth, we focus on rounding the $y$-values. To this end, we make the following useful definition.
\begin{definition}[Roundable Sets]\label{def:rnding-mkc}
	A set of facilities $S\subseteq F$ is said to be $(a,b)$-roundable w.r.t $(x,y)$ if
	\begin{itemize}[noitemsep]
		\item[(a)] $\diam_G(S) \leq a$
		\item[(b)] there exists a rounding $\y_{ip} \in \{0,1\}$ for all $i \in S, p\in [P]$ such that
		\begin{enumerate}
			\item $\sum_{q \geq p} \sum_{i\in S} \y_{iq} ~\leq~ \floor{\sum_{q \geq p}\sum_{i\in S} y_{iq}}$ for all $p$, and
			\item $\sum_{j\in C} d_j \sum_{i\in S,p\in [P]} x_{ijp} \leq b\cdot \sum_{i\in S} \sum_{p\in [P]} c_p \y_{ip}$
		\end{enumerate}
	\end{itemize}
\end{definition}
\noindent

\iffalse
If $(x,y)$ were feasible, then for any $(a,b)$-roundable set, we can integrally open facilities to satisfy all the demand that was fractionally assigned to it taking a hit of $a$ in the cost and a factor of $b$ in the capacities. Furthermore, the number of open facilities is at most what the LP prescribes. Therefore, if we would be able to decompose the instance into roundable sets, we would be done.
Unfortunately, that is not possible, and in fact the above LP has a large integrality gap even when we allow arbitrary violation of capacities.

\begin{remark}[Integrality Gap for \mckc] \label{rem:ig}
Consider the following instance. The metric space $X$ is partitioned into $(F_1\cup C_1) \cup \cdots \cup (F_K\cup C_K)$, with $|F_k| = 2$ and $|C_k| = K$ for all $1\le k\le K$.
The distance between any two points in $F_i\cup C_i$ is $1$ for all $i$, while all other distances are $\infty$. The capacities available are $k_1 = K$ facilities with capacity $c_1 = 1$ and
$k_2= K-1$ facilities with capacity $c_2 = K$. It is easy to see that integrally any solution would violate capacities by a factor of $K/2$.
%It is easy to see that the above instance is not feasible with $OPT=1$: indeed, there is at least one client location where the optimal solution does not place a facility of capacity $H$ in its neighborhood, and it is not possible to serve the demand of this client using only capacity $1$ facilities, as there are only two locations where we can place facilities in its neighborhood.
On the other hand, there is a feasible solution for the above LP relaxation: for $F_k = \{a_k,b_k\}$, we set $y_{a_k2} = 1-1/K$ and $y_{b_k1} = 1$, and for all $j\in C_k$, we set $x_{a_kj2} = 1-1/K$ and $x_{b_kj1} = 1/K$.


 For the version with soft capacities, we do not have the constraint \eqref{eq:lp5} and the above integrality gap doesn't hold since we can install capacity $K$ facilities on $K-1$ of the sets $F_k$'s, $1\leq k\leq K-1$, and $K$ copies of the capacity $1$ facilities at $F_K$. Note that although $|F_K| = 2$, we have opened $K$ capacities.
\end{remark}

In particular, note that for the $(x,y)$ solution in the integrality gap example above there are no roundable sets. This motivates the definition of the second kind of sets.
\fi

So if we can partition the facilities into roundable sets with reasonable parameters, we would be done.   It turns out that sets which are not roundable have a \emph{non-expanding structure}, and indeed we define our \cckp instance over such sets. The following definition comes handy in this case.

\begin{definition}[Complete Neighborhood Sets] \label{def:comp-nbr}
	A subset $T\subseteq F$ of facilities is called a {\em complete neighborhood} if there exist clients $J\subseteq C$ such that $\Gamma(J) \subseteq T$.
	In this case $J$ is said to be {\em responsible} for $T$. Additionally, a complete neighborhood $T$ is said to be an $\alpha$-complete neighborhood if $\diam(T) \leq \alpha$.
\end{definition}

%\begin{remark}[Complete Neighborhood Sets to \cckp]\label{rem:red}
%	\emph{
If we find a complete neighborhood $T$ of facilities with a set $J$ of clients responsible for it, then we know that the optimal solution \emph{must satisfy} all the demand in $J$ by suitably opening facilities of sufficient capacity in $T$.
Thus, if we can partition the entire instance into a collection $\calT = (T_1,\ldots,T_m)$ of disjoint $\alpha$-complete neighborhood sets with $J_i$ responsible for $T_i$, we can define an instance $\calI$ of \cckp with $m$ machines with demands $D_i = |J_i|$ and cardinality constraint $f_i = |T_i|$, and there are $n_i$ jobs of capacities $c_i$ for $1 \leq i \leq P$.

However, in general, our decomposition theorem only ensures that we can partition the instance into sets which are either roundable or are complete neighborhoods, and the crux of the rounding lies in combining the two cases while meeting the $k_i$ bounds for all capacities. Our next definition is that of $(\tau,\rho)$-{\em deletable clients} that can be removed from the instance since they can be ``$\rho$-charged'' to the remaining clients that are at most $\tau$-away.
\begin{definition}[Deletable Clients]\label{def:deletable}
	A subset $\Cd\subseteq C$ of clients is $\rho$-deletable if there exists a mapping $\phi_{j,j'}\in [0,1]$ for $j\in \Cd$ and $j'\in C\setminus \Cd$ satisfying (a) $\sum_{j'\in C\setminus \Cd} \phi_{j,j'} = 1$ for all $j\in \Cd$, and(b) $\sum_{j\in \Cd} \phi_{j,j'} \leq \rho$ for all $j'\in C\setminus \Cd$. Furthermore, $\phi_{j,j'} > 0$ only if $d(j,j') \leq \tau\cdot\opt$.



%The facilities opened by the $\opt $ solution corresponds to a valid solution for $\calI$; furthermore, any $\beta$-approximate solution for $\calI$ corresponds to a $(\alpha,\beta)$-approximate solution for the \mckc problem restricted to clients in $\cup_{\ell} J_\ell$. Finally note that for \mckc with soft-capacities, $\calI$ is an instance of the $Q||C_{min}$ problem.
%}

%\emph{
%Note that the above integrality gap  example is essentially a \cckp instance with $K$ machines of demand $K$ each having cardinality constraint $2$, and there are $K$ jobs of capacity $1$ and $K-1$ jobs with capacity $K$. This shows the assignment LP has bad integrality gap for the \cckp problem (but not for $Q||C_{min}$).}
%\end{remark}



\end{definition}
\iffalse
 The following claim shows we can remove $\Cd$ from consideration.
\begin{claim}\label{clm:prelim3}
	Let $\Cd$ be a $(\rho,\tau)$-deletable set.
	Given an $(a,b)$-approximate feasible solution $(x',\y)$ where $x'_{ijp}$ is defined only for $j\in C\setminus \Cd$, we can extend $x'$ to a general $(x,\y)$ solution
	which is $(a+\tau, b(1+\rho))$-approximate feasible.
\end{claim}
\begin{proof}
For any $j\in \Cd$, define $x_{ijp} = \sum_{j'\in C\setminus \Cd} x_{ij'p}\phi_{j,j'}$.
We get for all $j\in \Cd$,
$\textstyle \sum_{i\in F} \sum_{p\in [P]} x_{ijp} = \sum_{i,p} \sum_{j'\in C\setminus \Cd} x_{ij'p}\phi_{j,j'} = \sum_{j'\in C\setminus \Cd} \phi_{j,j'} \left(\sum_{i,p} x_{ij'p}\right) \geq \sum_{j'\in C\setminus \Cd} \phi_{j,j'} = 1$,
and for all $i\in F,p\in [P]$,
$\textstyle \sum_{j\in \Cd}  x_{ijp} = \sum_{j\in \Cd} \sum_{j'\in C\setminus \Cd} x_{ij'p}\phi_{j,j'} = \sum_{j'\in C\setminus \Cd} x_{ij'p}\left( \sum_{j\in \Cd} \phi_{j,j'}\right)  \leq \rho \sum_{j'\in C\setminus \Cd} x_{ijp} \leq b\rho c_p$. Therefore, in all we have $\sum_{j\in C} x_{ijp} \leq bc_p(1+\rho)$.
\end{proof}
\fi


Our final ingredient is that of supply polyhedra. Recall that an instance of  \cckp has $m$ machines $M$ with demands $D_1,\ldots,D_m$ and cardinality constraints $f_1,\ldots, f_m$, and $n$  jobs $J$ with capacities $c_1,\ldots,c_n$ respectively. Now, we generalize this in the following manner:
%In $Q||c_{min}$, there are no $f_i$'s, or equivalently $f_i = \infty$.
%In the version with cardinality constraints, that is $Q|f_i|C_{min}$ we are also given positive integers $f_1,\ldots, f_m$.
 A {\em supply vector} $(s_1,\ldots,s_n)$ where each $s_j$ is a non-negative integer
is called {\em feasible} for this instance if the ensemble formed by $s_j$ copies of jobs of capacity $c_j$ can satisfy all the demands.
The {\em supply polyhedra} then desires to capture these feasible supply vectors.

\begin{definition}[Supply Polyhedron]\label{def:supp-poly}
	Given an instance $\calI$ for a max-min allocation problem, a polyhedron $\calP(\calI)$ is called an $\alpha$-approximate supply polyhedron if
	(a) all feasible supply vectors lie in $\calP(\calI)$, and (b) given any non-negative integer vector $(s_1,\ldots,s_n)\in \calP(\calI)$ there exists an assignment
	of the $s_j$ jobs of capacity $c_j$ to the machines such that machine $i$ receives capacity $\geq D_i/\alpha$.
\end{definition}

Ideally, we would like {\em exactly} supply polyhedra, and one choice would be the convex hull of all the feasible supply vectors; indeed this is the tightest polytope satisfying condition (a).
Unfortunately, there are instances of \cckp where the convex hull contains infeasible integer points for which $\alpha = \Theta(\log n/\log \log n)$.


\section{\mckc via Supply Polyhedra}\label{sec:o1}
\def\yy{y^\calT}
In this section, we prove the following theorem. %One of the main engines will be our strong decomposition theorem (\Cref{thm:decomp}) which we will state here but will prove in the next section.
\begin{theorem}\label{thm:reduction}
Suppose there exists $\beta$-approximate supply polyhedra  for all instances of $Q|f_i|C_{min}$ (resp., $Q||C_{min}$) which have $\gamma$-approximate separation oracles.
Then for any $\delta\in(0,1)$, there is an $\left(\tilde{O}(1/\delta),\gamma\beta(1+5\delta)\right)$-bicriteria approximation algorithm for  \mckc (resp., with soft capacities).
\end{theorem}
\noindent
	
\noindent
\noindent
%
%As discussed in the Introduction, for the \mckc problem, the above LP has unbounded integrality gap (although, as we will see later, with soft capacities this is not the case).
%To obtain non-trivial algorithms we would need to strengthen the LP. Nevertheless, a feasible solution $(x,y)$ to LP~\eqref{eq:lp1}-\eqref{eq:lp6} gives us a way to decompose the problem
%into ``easily roundable parts'' and ``\cckp parts". To formalize this, we make two definitions.
%
%\begin{definition}\label{def:rnding-mkc}
%	A set of facilities $S\subseteq F$ is said to be $(a,b)$-roundable w.r.t feasible solution $(x,y)$ if
%	\begin{itemize}[noitemsep]
%		\item[(a)] $\diam_G(S) \leq a$
%		\item[(b)] there exists a rounding $Y_{ip} \in \{0,1\}$ for all $i \in S, p\in [P]$ such that
%		\begin{enumerate}
%			\item $\sum_{q \geq p} \sum_{i\in S} Y_{iq} ~\leq~ \floor{\frac{1}{2} \cdot \sum_{q \geq p}\sum_{i\in S} y_{iq}}$ for all $p$, and
%			\item $\sum_{j\in C} d_j \sum_{i\in S,p\in [P]} x_{ijp} \leq b\cdot \sum_{i\in S} \sum_{p\in [P]} c_p Y_{ip}$
%		\end{enumerate}
%	\end{itemize}
%\end{definition}
%\noindent
%For any $(a,b)$-roundable set, we can integrally open facilities to satisfy all the demand that was fractionally assigned to it taking a hit of $a$ in the cost and a factor of $b$ in the capacities.
%Furthermore, the number of open facilities is at most what the LP prescribes.
%%The idea behind the above definition should be clear.
%%Suppose $S$ is a set of facilities and consider a subset of demands $J$ which are being assigned (fractionally) by
%%the solution $(x,y)$ to $S$. If $S$ is $(a,b)$-roundable wrt $(x,y)$, then we can open facilities in $S$ integrally and reassign the demands in $J$ to these integral
%%facilities. By doing so, we shall increase the connection cost of demands in $J$ by an additive factor of $a$, and then we may violate the capacities of the integrally open
%%facilities by at most a factor $b$.
%\begin{definition} \label{def:comp-nbr}
%	A subset $S\subseteq F$ of facilities is called a {\em complete neighborhood} if there exists a client-set $J\subseteq C$ such that $\Gamma(J) \subseteq S$.
%	In this case the subset $J$ is said to be {\em responsible} for $S$. Additionally, a complete neighborhood $S$ is said to be an $a$-complete neighborhood if $\diam(S) \leq a$.
%\end{definition}
%\noindent
%%In a complete neighborhood set $S$ with $J$ responsible for it, we must open a total capacity of at least $|J|$ units among facilities in $S$.
%%A collection of disjoint complete neighborhood sets therefore correspond to a \cckp instance. If the diameter of each set is $\leq \alpha$, then $\beta$-approximate solutions to the
%%\cckp instance correspond to $(\alpha,\beta)$-bicriteria approximation.
%If we find a complete neighborhood $S$ of facilities with say a set $J$ of clients responsible for it, then we know that the optimal solution must satisfy all the demand in $J$ by suitably opening facilities of sufficient capacity in $S$. A disjoint collection of such complete neighborhoods leads to a \cckp problem instance. % described in Idea 1.
%\smallskip
%
%\noindent
Our results for \mckc follow from \Cref{thm:reduction} and results about supply polyhedra.
For example, Theorem~\ref{thm:2} follows from~\Cref{thm:reduction} (using $\delta=0.5$, say) and Theorem~\ref{thm:conflp}, and also noting that $D_\mathrm{max}/D_\mathsf{min} \leq n$ in our reduction. %Theorem~\ref{thm:2a} follows
%from~\Cref{thm:reduction,thm:asslp}.
We now state our decomposition result using which we prove~\Cref{thm:reduction}. %which essentially states that given an \mckc instance, we can partition the problem into roundable and complete neighborhood sets. The reader may want to recall the definitions of roundable sets (Definition~\ref{def:rnding-mkc}), complete neighborhood sets (Definition~\ref{def:comp-nbr}), deletable sets (Definition~\ref{def:deletable}), and the natural LP relaxation \eqref{eq:lp1}-\eqref{eq:lp6}.
%Our main techincal theorem is the following
%It is perhaps instructive to compare the below theorem with Theorem~\ref{thm:weakdecomp}.
%The proof of this theorem is rather technical, and we defer it to the next section.
\begin{theorem}[{\bf Decomposition Theorem}]\label{thm:decomp}
	Given a feasible solution $(x,y)$ to LP\eqref{eq:lp1}-\eqref{eq:lp6}, and $\delta > 0$, there is a polynomial time algorithm which finds a solution $\x$ satisfying \eqref{eq:lp2} and\eqref{eq:lp4}, and a
	decomposition as follows.
	\begin{enumerate}%[noitemsep]
		\item The facility set $F$ is partitioned into two families $\calS = (S_1, S_2, \ldots, S_K)$ and $\calT = (T_1, T_2, \ldots, T_L)$ of mutually disjoint subsets.
		The client set $C$ is partitioned into three disjoint subsets $C = \Cd \cup \Cbb \cup \Cb$ where $\Cd$ is a $(\tilde{O}(1/\delta),\delta)$-deletable subset.
		
			\item Each $S_k \in \calS$ is $(\tilde{O}(1/\delta),(1+\delta))$-roundable with respect to $(\x,y)$, and moreover, each client in $\Cb$ satisfies $\sum_{i \in \calS, p} \x_{ijp} \geq 1 - \frac{\delta}{100}$.
%\comment{deepc: maybe we should make 100 less arbitrary}
		\item Each $T_\ell$ is a $\tilde{O}(1/\delta)$-complete neighborhood with a corresponding set $J_\ell$ of clients responsible for it, and $\Cbb = \cup_{\ell = 1}^L J_\ell$.	
%		
%		
%		\item For the deleted clients $\Cd$, there is a mapping $\phi:\Cd \to \Cbb \cup \Cb$ such that
%		(a) $d(j,\phi(j)) \leq \tilde{O}(1/\delta)$ for all $j\in \Cd$, and
%		(b)	for all $j\in \Cbb \cup \Cb$, we have $\sum_{j' \in \Cd: \phi(j') = j} d_{j'} \leq (1+\delta)\cdot d_j$, i.e., the total demand mapped to $j$ is small.
%		
	\end{enumerate}
\end{theorem}


\begin{proof}[{\bf Proof Sketch of Theorem~\ref{thm:reduction}}]
Let us first describe an approach which fails. Let $(x,y)$ be a feasible solution to LP\eqref{eq:lp1}-\eqref{eq:lp6}, and apply~\Cref{thm:decomp}.
Although the sets in $\calS$ by definition are roundable which takes care of the clients in $\Cb$, the issue arises in assigning clients of $\Cbb$.
In particular, $\yy_p := \sum_{i\in \calT} y_{ip}$ for all $1\le p\le P$ which indicates the ``supply" of capacity $c_p$ available for the $\Cbb$ clients.
%Since the LP doesn't know $\calT$ beforehand, this supply mayn't be enough.
However, this may not be enough for serving all these clients (even with violation).
That is, the vector $\yy$ may not lie in the (approximate) supply polyhedra of the \cckp instance
defined by $\calT$. % as described in Remark~\ref{rem:red}.
 That we fail is not surprising; after all, we have so far only used the natural LP which has a bad integrality gap. To resolve this issue, we strengthen the LP by {\em explicitly requiring $\yy$ to be in the supply polyhedra}. Since we do not know $\calT$ before solving the LP (after all our LP rounding generated it), we enforce this for {\em all} collections of complete-neighborhood sets.
More precisely, for $\calT := (T_1,\ldots,T_L)$ of $L$ disjoint complete neighborhood sets, let $\calI_\calT$ denote the associated \cckp demands.
\begin{equation}\label{eq:lp7}
\forall \calT := (T_1,\ldots,T_L) \textrm{ disjoint neighborhood subsets}, \quad \yy \in \calP(\calI_\calT) \tag{\small{L7}}
\end{equation}
Note that this is a feasible constraint to add to LP\eqref{eq:lp1}-\eqref{eq:lp6}. In the $\opt$ solution, for any $\calT$ there must be enough supply dedicated for the clients responsible for these complete neighborhood sets.  We don't know how (and don't expect) to check feasibility of  \eqref{eq:lp7} for all collections $\calT$. However, we can still run ellipsoid method using the ``round-and-cut'' framework of \cite{CarrFLP00,ChakrabartyCKK11,Li15,Li16}.
To begin with, we start with the LP\eqref{eq:lp1}-\eqref{eq:lp6} and obtain feasible solution $(x,y)$. Subsequently, we apply the decomposition Theorem~\ref{thm:decomp} to obtain the collection $\calT = (T_1,\ldots,T_L)$.
We then check if $\yy \in \calP(\calI_\calT)$ or not. Since we have a $\gamma$-approximate separation oracle for $\calP(\calI_\calT)$, we  are either guaranteed that $\yy \in \calP(\calI'_\calT)$ where the $\ell^{th}$ demand is now  $D_\ell/\gamma$; or we get a hyperplane separating $\yy$ from $\calP(\calI_\calT)$ which also gives us a
hyperplane separating $y$ from  LP\eqref{eq:lp1}-\eqref{eq:lp7}. This can be fed to the ellipsoid algorithm to obtain a new  $(x,y)$ and the above process is repeated.

When this process stops, we will have a solution $(x,y)$ such that the supply $\{y_p^{\calT}\}$ lies in the supply polyhedra $\calP(\calI_\calT)$. So our overall algorithm is to simply round the roundable sets (by rounding down), and solve the instance $\calI_\calT$ with the supply vector $\{y_p^\calT\}$ using a suitable \cckp algorithm.
\end{proof}

We end the main body by noting that the configuration LP relaxation is in fact nearly the best possible supply polyhedra for \cckp.

\begin{theorem}\label{thm:conflp}
	For any instance $\calI$ of \cckp, the natural configuration LP for $\calI$ is an $O(\log D)$-approximate supply polyhedron with $(1+\epsilon)$-approximate separation oracle for any $\eps > 0$,
	where $D := D_{\mathrm{max}}/D_\mathrm{min}$. Moreover, there exists no supply polyhedra with approximation $o(\log D/\log \log D)$.
%	Given $(s_1,\ldots,s_n) \in \calP_\mathsf{conf}$ for an instance $\calI$ of $Q|f_i|C_{min}$, there is an of assignment of the $s_j$ jobs of capacity $c_j$  to the machines such that for all $i\in M$
%	receives a total capapcity $\geq D_i/\alpha$ for $\alpha = O(\log D)$ where $D = D_{max}/D_{min}$.
\end{theorem}


\iffalse
The analysis of the ellipsoid algorithm\comment{deepc: need to be careful and correct here}
tells us that in polynomial time we either prove infeasibility of the system \eqref{eq:lp1}-\eqref{eq:lp7} (implying the $\opt$  guess for \mckc is infeasible), or we
are have $(x,y)$ satisfying the premise of the following lemma.
%obtain a solution $(x,y)$
%which is feasible for LP\eqref{eq:lp1}-\eqref{eq:lp6}, such that for the $\calS, \calT$ obtained via Decomposition Theorem~\ref{thm:decomp}
%and the instance $\calI_\calT$ so obtained, the solution  $\yy \in \calP(\calI'_\calT)$ for the $\gamma$-shaded instance.

\begin{lemma}
	Given $(x,y)$ feasible for  LP\eqref{eq:lp1}-\eqref{eq:lp6}, let us apply the Decomposition Theorem~\ref{thm:decomp} to obtain the instance $\calS,\calT$.
	Suppose the solution $\yy_p := \sum_{i\in\calT} y_{ip}$ lies in $\calP(\calI'_\calT)$ for the \cckp (respectively, $Q||C_{min}$) instance $\calI'_\calT$ with $L$ machines with $D_\ell := |J_\ell|/\gamma$
	and $f_\ell := |T_\ell|$ (respectively, no cardinality constraints). Then we can obtain an $(\tilde{O}(1/\delta), \beta\gamma(1+\delta))$-approximate solution to the \mckc problem (respectively, with soft-capacities).
\end{lemma}
\begin{proof}
%Suppose the latter occurs. From this we can obtain the bicriteria solution to the \mckc problem as follows.
%Recall the notation in the Decomposition Theorem~\ref{thm:decomp}.
Since every set $S_k, 1\leq k\leq K,$ is $(\tilde{O}(1/\delta),(1+\delta))$-roundable, there exists a rounding $\y_{ip}$ for $i\in S_k$  such that
\begin{equation}\label{eq:repeat}
\textstyle \forall p, ~~~ \sum_{q\geq p} \sum_{i\in S_k} \y_{iq} \leq \floor{\sum_{q\geq p} \sum_{i\in S_k} y_{iq}}
\end{equation}
\def\s{\tilde{s}}
Ideally, we would like to open a facility of capacity $c_p$ at location $i$ whenever $\y_{ip} = 1$. Unfortunately, the decomposition theorem doesn't have capacity constraints for individual $p$'s but only their suffix sums. Instead we do the following. Define $y^{\calS}_p := \sum_{i\in \calS} y_{ip}$; LP\eqref{eq:lp3} implies that for all $p$, $y^\calS_p + y^\calT_p \leq k_p$.
For $1\leq p\leq P$, define $s_p := \sum_{i\in \calS} \y_{ip}$; \eqref{eq:repeat} implies for all $p$, $\sum_{q\geq p} s_q \leq \floor{\sum_{q\geq p} y^\calS_q}$ (since $\floor{a} + \floor{b} \leq \floor{a+b}$.)
\begin{claim}\label{clm:massmovement}
	Given $(s_1,\ldots,s_P)$ satisfying $\sum_{q\geq p} s_q \leq \floor{\sum_{q\geq p} y^\calS_q}$, there exists $(\s_1,\ldots,\s_P)$ satisfying
	for all $p$, (a) $\sum_{q\geq p} s_q \leq \sum_{q\geq p} \s_q \leq \sum_{q\leq p} y^\calS_q$, and (b) $\s_p \leq k_p$.
\end{claim}
\begin{proof}
Simply define $\s_p := \floor{\sum_{q\geq p} y^\calS_q} - \floor{\sum_{q> p} y^\calS_q}$. Therefore, $\sum_{q\geq p} \s_q = \floor{\sum_{q\geq p} y^\calS_q}$ implying (a).
To see (b), note $\s_p \leq \ceil{y^\calS_p} \leq k_p$, where we use the fact $\floor{a+b} \leq \floor{a} + \ceil{b}$ for any non-negative $a,b$.
\end{proof}

The first inequality in (a) implies that at every location with $\y_{ip} = 1$, we can open a facility of capacity $c_q \geq c_p$. This, along with condition (b) of roundable sets (Definition~\ref{def:rnding-mkc}),
implies we can find a fractional solution $x_{ijp}$ for $j\in \Cb$ and $(i,p)$ with $\y_{ip} = 1$
such that (a) $\sum_{i\in \calS, p\in [P]} x_{ijp} \geq 1$, (b) $x_{ijp} > 0$ only if $d(i,j) \leq \diam(S_k) \leq \tilde{O}(1/\delta)$, and (c) the capacity violation is $\leq (1+\delta)(1 - \delta/100)^{-1} \leq (1+2\delta)$. Note the second term arises since
from the decomposition theorem we have $\sum_{i\in \calS, p\in [P]} \x_{ijp} \geq 1-\delta/100$.
Thus we have fractionally assigned all $\Cb$ clients to open facilities in $\calS$.
%For all $j\in \Cb$, we assign it fractionally using $\frac{\x}{1-\delta/100}$ to


Define, for $p\in [P]$,  $t_p := k_p - \s_p$, the number of facilities of capacity $c_p$ we can open in $\calT$. Note, by Claim~\ref{clm:massmovement}, $t_p$'s are non-negative.
%
%
\begin{claim}
	$(t_1,\ldots,t_P) \in \calP(\calI'_\calT)$
\end{claim}
%	We now use the upward-feasibility property of $\calP$ to prove that the integral vector $(k^{(T)}_1,\ldots, k^{(T)}_P)$ also lies in $\calP(\calI'_\calT)$.
\begin{proof}
	By the Lemma premise, we have $\yy \in \calP(\calI'_\calT)$. %Using the upward-feasibility property of $\calP$, we get the following.
	%Recall that $\calI'_\calT$ has $L$ machines with demands $D_\ell := |J_\ell|/\beta$ and $f_\ell := |T_\ell|$.
	Now note that for all $p$,
	\[
\textstyle 	\sum_{q\geq p} t_q = \sum_{q\ge p} (k_q - \s_q) \ge \sum_{q\ge p} k_q - \sum_{q\geq p} y^\calS_q \geq  \sum_{q\geq p} y^\calT_q
	\]
	Since $\calP(\calI'_\calT)$ is upward-feasible, and $\yy\in \calP$, we get the claim.
\end{proof}
Since $\calP(\calI'_\calT)$ is $\beta$-approximate, we can find an allocation of the $t_p$ copies of jobs of capacity $c_p$ to the $L$ machines of $\calI'_\calT$ such that machine $\ell$ gets at most $f_\ell$ jobs and total capacity $\geq D_\ell/\beta = |J_\ell|/\beta\gamma$. We install these capacities on the facilities of $T_\ell$. Since the diameter of each $T_\ell$ is $\tilde{O}(1/\delta)$, we can find an $x_{ijp}$ assignment of $\Cbb$-clients  to these such that $\sum_{i\in \calT,p\in [P]} x_{ijp} \geq 1$ and $x_{ijp} > 0$ iff $d(i,j) = \tilde{O}(1/\delta)$, such that the capacity violation is at most $\alpha\beta$. This takes care of the clients in $\Cbb$. Finally, Claim~\ref{clm:prelim3} takes care of all the deleted clients $\Cd$ with an extra hit of $(1+\delta)$ on the capacity and additive $\tilde{O}(1/\delta)$ on the distance.
\end{proof}
\noindent
This completes the proof of Theorem~\ref{thm:reduction} for the general \mckc problem. For the problem with soft capacities, the proof is exactly the same, except in the end, the instance $\calI_\calT$ is a $Q||C_{min}$ instance rather than a \cckp one.
\end{proof}


We end this section by noting that for the \mckc problem with soft-capacities, if we use the assignment supply polyhedra described in Section~\ref{sec:supplypolyhedra}, then we do not need to run the ellipsoid algorithm.
In particular, the inequality \eqref{eq:lp7} is implied \eqref{eq:lp1}-\eqref{eq:lp6} for $\calP_\mathsf{ass}$ defined in \eqref{eq:asslp1}-\eqref{eq:asslp3}.
\begin{lemma}\label{lem:implied}
Given any $(x,y)$ feasible for LP\eqref{eq:lp1}-\eqref{eq:lp6} and any $\calT = (T_1,\ldots,T_m)$, we have $\yy \in \calP_\mathsf{ass}(\calI_\calT)$.
\end{lemma}
\begin{proof}
	Fix $\calT = (T_1,\ldots,T_m)$ to be a collection of complete neighborhood sets. In the instance $\calI_\calT$ of $Q||C_{min}$, we have $m$ machines with demands
	$D_\ell = |J_\ell|$, where $J_\ell$ is the client set responsible for $T_\ell$. Recall, $y^\calT_p := \sum_{i \in \calT} y_{ip}$, and we need to find $z_{\ell,p}$ which satisfy the constraints
	\eqref{eq:asslp1}-\eqref{eq:asslp3} where $s_p := y^\calT_p$.
	
	The definition is natural: $z_{\ell,p} := \sum_{i\in T_\ell} y_{ip}$. Clearly it satisfies \eqref{eq:asslp1} (indeed with equality). We now show it satisfies \eqref{eq:asslp2}.
	To this end, define for any $j\in J_\ell$, $x_{jp} := \sum_{i\in T_\ell} x_{ijp}$. Since $\Gamma(J_\ell) \subseteq T_\ell$, we get from \eqref{eq:lp1} that $\sum_p x_{jp} \geq 1$.
	In particular,
	\begin{equation}
\textstyle 	\label{eq:hohum1}\sum_p \sum_{j\in J_\ell}x_{jp} \geq D_\ell
	\end{equation}
	
	From \eqref{eq:lp4}, we know $x_{ijp} \leq y_{ip}$ and summing over all $i\in T_\ell$, we get for all $j\in T_\ell$, $x_{jp} \leq \sum_{i\in T_\ell} y_{ip} = z_{\ell,p}$.
	In particular, $\sum_{j\in J_\ell} x_{jp} \leq z_{\ell,p} D_\ell$. From \eqref{eq:lp2} we know for all $i\in T_\ell, p\in [P]$, $\sum_{j\in J_\ell} x_{ijp} \leq c_p y_{ip}$.
	Summing over all $i\in T_\ell$, gives $\sum_{j\in J_\ell} x_{jp} \leq c_p z_{\ell,p}$. Putting together, we get
	\begin{equation}
	\textstyle 	\label{eq:hohum2}\sum_{j\in J_\ell}x_{jp} \leq z_{\ell,p} \min(D_\ell,c_p)
	\end{equation}
	\eqref{eq:hohum1} and \eqref{eq:hohum2} imply that $z$ satisfies \eqref{eq:asslp2}.
\end{proof}
Therefore, one can use the natural LP relaxation to obtain for any $\delta > 0$, a $\left(\tilde{O}(1/\delta),(2+\delta)\right)$-bicriteria approximation for the \mckc problem with soft capacities.
As it should be clear, this is a much more efficient algorithm.

\fi



% described in Idea 1.







==> section1.tex <==
\section{Introduction}
The capacitated $k$-center problem is a classic optimization problem where a finite metric space $(X,d)$ needs to be partitioned into $k$ clusters so that  every  cluster has cardinality at most
some specified value $L$, and the objective is to minimize the maximum intra-cluster distance. This problem was introduced by Bar-Ilan et al~\cite{Bar-IlanKP93} and has many applications~\cite{LuptonMY98,MorganL77,Murthy1983AnAA} such as resource allocation in networks (e.g., where to place servers to minimize the total load and client latency), vehicle routing, etc. %see khuller-sussmann paper for these refs.
%{\em machine placement problem}: determine where to place a given collection of \emph{identical servers} to minimize the makespan (jobs are located in a metric space, and first need to reach the server they are assigned to before they can be processed). %\mcomment{Add Venkat's References?}
 The basic problem is {\em homogeneous} in the sizes of the clusters, that is, it has the same cardinality constraint $L$ for each cluster. In certain applications however, a \emph{heterogeneous} version of the problem where we have different cardinality constraints for the clusters might be more applicable.
For example, consider the following problem: given a set of demands/clients in a network, and a collection of heterogeneous machines/servers of different capacities, where do we place the servers and how do we assign the clients to servers so that machine capacities are respected and the maximum client-server distance is minimized. %We could possibly load higher-speed machines with more jobs than lower-speed ones.
Motivated by such applications, we study the worst-case complexity of this heterogenous version in this paper.

\begin{definition}\emph{(The \mckc Problem\footnote{Technically, we should call our problem the Heterogeneous Capacitated $k$-Supplier Problem since we can only open centers in $F$. However, we avoid making this distinction throughout this paper.}.)}
	%	\begin{itemize}[noitemsep]
	%		\item {\bf Input:} Metric space $\left(X=F\cup C, d\right)$ where $F$ are facilities and $C$ are clients.
	%		\\$~~~~~~~~~~$ Collection: $(k_1,c_1), \ldots, (k_P,c_P)$ of $P$-tuples of positive integers.
	%		\item {\bf Output:} $F_1,\ldots, F_P \subseteq F$ which are pairwise disjoint and $|F_p| \leq k_p$ for all $1\le p\leq P$. \\
	%		$~~~~~~~~~~~~$ Assignment $\phi: C\to F_1\cup F_2\cup \cdots \cup F_P$ such that for all $p$, $|\{j\in C: \phi(j)\in F_p\}|\leq c_p$.
	%		\item {\bf Objective:} Minimize $\max_{j\in C} d(j,\phi(j))$.
	%	\end{itemize}
	We are given a metric space $(X = F\cup C,d)$  where $C$ and $F$ represent the clients and facility locations.%where the set $X$ is partitioned into facilities $F$ and clients $C$.
	%Furthermore, the input contains
	We are also given a collection of {\em heterogeneous} capacities: $(k_1,c_1), (k_2,c_2),\ldots, (k_P,c_P)$ with $k_i$ copies of capacity $c_i$.
	%with $c_1 \leq c_2 \le \cdots \le c_t$,  to indicate we can open $k_p$ centers (called type $p$ centers) with capacity $c_p$ in $F$.
	The objective is to install these capacities at unique locations $F'\subseteq F$, and find an assignment $\phi:C\to F'$ of clients to these locations,
	such that for any $i\in F'$ the number of clients $j$ with $\phi(j) = i$ is at most the capacity installed at $i$, and $\max_{j\in C} d(j,\phi(j))$ is minimized.
%	The objective is to minimize
	%
	% to open these centers and assign all points of $C$ to one of these so that (a) any center of type  $p$ serves at most $c_p$ clients, and (b) the maximum distance of a client $j$ to its assigned center $i$ is minimized.
%	We use $\opt$ to denote this latter distance of the optimum solution.
	A weaker version, which we call \mckc  with soft capacities, allows multiple capacities to be installed at the same location.
\end{definition}
\noindent
Note that when all $c_p = L$ and $\sum_p k_p = k$, we get back the usual capacitated $k$-center problem.
The \mckc problem is relevant in many applications where the resources available are heterogenous. The machine placement problem is one example which has applications in network scheduling~\cite{QiuSZ15,ImM15a} and distributed databases~\cite{MorganL77,SKRN15}. Another example is that of  vehicle routing problems with  fleets of different speeds~\cite{GortzMN016}. A third relevant application may be clustering; often clusters of equal sizes are undesirable~\cite{GuhaRS01} and explicitly introducing heterogeneous constraints might lead to desirable clusters.

For the homogeneous (uniform capacities) problem, Bar-Ilan et al~\cite{Bar-IlanKP93} gave a $10$-approximation which was improved to a $6$-factor approximation by Khuller and Sussmann~\cite{KhullerS00}. One cannot get a better than $2$-approximation even for the {\em uncapacitated} $k$-center problem~\cite{HochbaumS85}. Recently, some works~\cite{CyganHK12,AnBCGMS14} study the {\bf non-uniform capacitated $k$-center problem} and get constant-factor approximations: in this problem, every facility location $v\in F$ has a \emph{pre-determined} capacity $c_v$ if opened (and $0$ otherwise), and the objective is again to minimize the maximum distance of a client to its assigned open facility while opening $k$ facilities. We remark that the non-uniform version and our heterogeneous version seem unrelated in the sense that none is a special case of the other, and moreover, they present different sets of technical challenges to overcome.

\subsection{Main Results}

As mentioned above, both the uniform and the non-uniform capacitated $k$-center problems described above admit $O(1)$-approximation. In contrast, we show using a simple reduction that, assuming $P \neq NP$, \emph{no non-trivial approximation exists} for even the soft-version of \mckc, unless we {\em violate the capacities}. This observation (a) highlights the technical differences between our problem and these versions studied previously, and (b) motivates us to look at \emph{bicriteria approximations}: an $(a,b)$-approximation approximates the distance objective by a factor of $a$, while violating capacities by a factor of $b$.

%Although bicriteria approximation algorithms may be unsatisfactory, sometimes these can give unicriteria approximations for other related problems.
%We mention one application that  we alluded to above, and in fact was the starting point of this research,  which may be of independent interest.
%\begin{definition}\emph{(Machine Placement Problem for Network Scheduling.)}\label{def:mpp}
%	The input is a metric space $(X=F\cup C,d)$ with jobs with processing times $p_j$ at locations $C$. We are also given $P$ machines with speeds $s_1,s_2,\ldots,s_P$.
%	The goal is to find a placement of these machines on $F$ and schedule the jobs on these machines so as to minimize the makespan. The completion time of a job equals the time to reach the machine plus the processing time. In the ``soft" version of the problem, multiple machines may be placed in the same location.
%\end{definition}
%Although we do not prove it in this paper, any $(a,b)$-bicriteria approximation algorithm for (soft) \mckc problem implies an $O(a+b)$ approximation for the (soft) machine placement problem.

%The reduction in Remark~\ref{rem:cckp} does not rule out arbitrarily small violations to the capacity. Indeed the $Q||C_{min}$ problem has a PTAS~\cite{AzarE98}.
\begin{theorem}\label{thm:1}
	Fix an $\eps > 0$. There exists an $(O(\log n/\eps), (1+\eps))$-bicriteria approximation algorithm for the \mckc problem running in time $C_\eps^{\tilde{O}(\log^3n)}$ for a constant $C_\epsilon$ depending only on $\epsilon$. For \mckc with soft capacities, there exists an $(O(\log n/\eps), (1+\eps))$-bicriteria approximation algorithm running in time $n^{O(1/\epsilon)}$.
\end{theorem}

We prove the above theorem by reducing the \mckc problems to a class of {\em max-min allocation problems} for which we design good algorithms (details appear below). Our next set of results, which also forms one of the main technical contributions of the paper, aims at reducing the logarithmic factor in the approximation to the distance. %We can give $O(1)$-approximations if the violations are allowed to be $O(1)$ in the soft-capacity case and $O(\log n)$ in the general case.
%These algorithms run in polynomial time.
\begin{theorem}\label{thm:2}
	%For any $\eps > 0$, there exists an $\left(\tilde{O}(1/\eps), (1+\eps)\right)$-bicriteria approximation algorithm for \mckc which runs in time $n^{\tilde{O}\left(\frac{\log n}{\eps}\right)}$.
	There is a polynomial time  $(O(1),O(\log n))$-bicriteria approximation algorithm for the \mckc problem.
\end{theorem}
\begin{theorem}\label{thm:2a}
	%For any $\eps > 0$, there exists an $\left(\tilde{O}(1/\eps), (1+\eps)\right)$-bicriteria approximation algorithm for \mckc which runs in time $n^{\tilde{O}\left(\frac{\log n}{\eps}\right)}$.
	For any $\delta>0$, there is a polynomial time  $(\tilde{O}(1/\delta),2+\delta)$-bicriteria approximation for \mckc problem with soft capacities.
\end{theorem}
%\begin{corollary}
%There is a polynomial time $O(\log n)$ (resp. $O(1)$) approximation for non-uniform machine placement (resp. with machine co-location allowed).
%\end{corollary}
%In particular we have polynomial time $O(1)$ and $O(\log n)$ approximation algorithms for the machine placement problem of Definition~\ref{def:mpp}.


\subsubsection*{Connection to Non-Uniform Max-Min Allocation Problems.}
One main finding of this paper is the connection of \mckc~to the {\em non-uniform} max-min allocation (also known as Santa Claus~\cite{BansalS06}) problem. %thereby
 %underscoring the technical difficulty and difference of \mckc from  homogeneous (and also non-uniform) capacitated $k$-center. %we relate it to the classic $3$-Partitioning problem~\cite{Garey-Johnson}: in this problem
We now define these max-min allocation problems using  scheduling parlance.

\begin{definition}[$Q||C_{min}$ and \cckp]
In the\footnote{(Ab)using Graham's notation} $Q||C_{min}$ problem, one is given $m$ machines with demands $D_1,\ldots,D_m$ and $n$ jobs with capacities $c_1,\ldots,c_n$,
and the objective is to find an assignment of the jobs to machines satisfying each demand.
%We call this problem, (ab)using Graham's notation as $Q||C_{min}$.
In the {\em cardinality constrained}  non-uniform max-min allocation problem, denoted as the \cckp problem, each machine further comes with a cardinality constraint $f_i$, and a feasible solution cannot allocate more than $f_i$ jobs to machine $i$. The objective remains the same. An $\alpha$-approximate feasible solution assigns each machine $i$  total capacity at least $ D_i/\alpha$.
\end{definition}
\noindent

To show one side of the connection, we sketch how these problems arise as special cases
of \mckc, even with soft capacities.
\begin{remark}[Reduction from $Q|f_i|C_{min}$]\label{rem:cckp}
	Given an instance $\calI$ of $Q|f_i|C_{min}$, construct the instance of \mckc as follows. The capacities available to us are precisely the capacities of the jobs in $\calI$. The metric space is divided into $m$ groups $(F_1\cup C_1),\ldots,(F_m\cup C_m)$ such that the distance between nodes in any group is $0$ and across groups is $1$. Furthermore, for $1\leq i\leq m$, $|F_i| = f_i$ and $|C_i| = D_i$. Observe that the \mckc instance has a $0$-cost, capacity-preserving solution iff $\calI$ has a feasible assignment.
%	When there are soft capacities, the above reduction is from $Q||C_{min}$.
\end{remark}

Indeed, the strong NP-hardness\footnote{A simple reduction from 3-dimensional matching shows NP-hardness of \cckp and $Q || C_{min}$ even when the demands and capacities are polynomially bounded.} of \cckp and $Q || C_{min}$ shows that we cannot get true approximations for \mckc, with or without soft-capacities.
As mentioned before, our main technical contribution is in showing a connection in the converse direction as well. Indeed, our algorithms in~\Cref{thm:1,thm:2,thm:2a} use the following results we obtain for $Q|f_i|C_{min}$ and $Q||C_{min}$.

%We are not aware of non-trivial results for the \cckp problem (although, see Remark~\ref{rem:cckp-prev} below). We therefore call out the special case of the above theorem.
%This makes it rather improbable for \cckp to be APX-hard, and we leave the design of a PTAS as a challenging open problem.
\begin{theorem}\label{thm:q}
	There is a QPTAS for the \cckp problem.
\end{theorem}


%Once again, we call out what we believe is the first polynomial time non-trivial approximation to \cckp.
\begin{theorem}\label{thm:cckp}
	There is a poly-time logarithmic approximation algorithm for \cckp.
\end{theorem}

\begin{theorem} \label{thm:cckp-soft}
 There is a simple greedy $2$-approximation algorithm for $Q || C_{min}$.
 \end{theorem}

%We end the section by stating what we believe was the frontier of knowledge for the \cckp problem.
%\begin{remark}[Known algorithms for \cckp]\label{rem:cckp-prev}\emph{
	To our knowledge, \cckp has not been explicitly studied in the literature. % though the min-max version has been
	However, in a straightforward manner one can reduce \cckp to {\em non-uniform}, restricted-assignment max-min allocation problem (which we denote as $Q|restr|C_{min}$) where,  instead of the cardinality constraint dictated by $f_i$, we restrict jobs to be assigned only to a subset of the machines.\footnote{
	The reduction proceeds as follows: for every machine $i$ and job $j$, restrict $j$ to be assigned to $i$ iff $c_j \geq D_i/2f_i$. It is not hard to see that a $\rho$-approximation for the $Q|restr|C_{min}$ implies a $2\rho$-approximation for the \cckp instance.} Clearly $Q|restr|C_{min}$  is a special case of the general max-min allocation problem~\cite{ChakrabartyCK09} and therefore for any $\epsilon>0$, there are $n^{O(1/\epsilon)}$-time algorithms
achieving $O(n^\epsilon)$-approximation. We do not know of any better approximations for $Q|restr|C_{min}$. The {\em uniform} version $P|restr|C_{min}$ where all demands are the same~\cite{BansalS06} has a $O(1)$-approximations~\cite{Feige08,AsadpourFS12,PolacekS16}. However all these algorithms use the configuration LP, which unfortunately has an integrality gap of $\Omega(\sqrt{n})$ for the non-uniform version $Q|restr|C_{min}$ (see Appendix~\ref{sec:app-bsig} for the details.)%}
%\end{remark}


%%Although the violation in the capacities is large (although bounded by a constant), it already implies $O(1)$-approximations for the machine placement problem alluded to in the first paragraph.
%%This maybe of independent interest.
%\begin{theorem}\label{thm:mpp}
%	There is a polynomial time $O(1)$-approximate algorithm for the machine placement problem.
%\end{theorem}

%The reduction from $3$-Partitioning does not rule out non-trivial approximation algorithms which violate the capacity by $(1+\epsilon)$-factor for arbitrarily small $\epsilon>0$.
%Indeed, for $3$-Partitioning, there exist algorithms~\cite{bibid} which either return No, or find a partition with $\sum_{j\in S_i} a_j \geq D(1-\eps)$. %Thus for \mckc, approximation algorithms with  arbitrarily small capacity violation is not ruled out by the above reduction.
%However, as we discuss below, many {\em cardinality constrained scheduling problems} are also special cases of the \mckc problem. There are currently no PTASes known for these problems
%and in a sense which we elaborate in Section~\ref{sec:techs} capture the difficulty in the problem.
%Nevertheless, we are able to obtain non-trivial algorithms with $(1+\epsilon)$-capacity violation.
%
%%Our first result is an algorithm which for any $\eps>0$ returns an assignment which violates the capacities by at most $(1+\eps)$-factor and has cost at most $\tilde{O}(1/\eps)$ times $\opt$. However, it runs in quasipolynomial time.
%\begin{theorem}\label{thm:1}
%	For any $\eps > 0$, there exists an $(O(\log n/\eps), (1+\eps))$-bicriteria approximation algorithm for the \mckc problem running in time $C_\eps^{\tilde{O}(\log^3n)}$ for a constant $C_\epsilon$ depending only on $\epsilon$.
%	%There is an $(O(1),O(1))$-bicriteria approximation algorithm for the \mckc problem.
%\end{theorem}
%%When restricted to polynomial time algorithms, we can get constant factor approximations.
%%
%%As of now we do not know whether there are $(O(1),(1+\eps))$-bicriteria approximation algorithms for the \mckc problem -- we leave this as an open problem in our paper.
%%However, for this to exist, one must first obtain PTASes for certain {\em cardinality constrained scheduling} problems looked at the literature, for which only constant factor algorithms are currently known.
%%
%%We end this section with two comments.

%We encapsulate this in the following theorem.
%
%\begin{theorem}
%	Any algorithm for \mckc violating the capacity constraints by $(1+\eps)$ would imply a PTAS for cardinality constrained max-min allocation problem on uniform speed machines.
%	%Any $(a,b)$-bicriteria approximation for \mckc implies a $b$-approximation for the cardinality constrained max-min allocation problem on uniform speed machines.
%\end{theorem}
%\noindent
%One of the main components of our algorithm for \mckc is a constant-approximation for $Q|k_i|C_{min}$. We call out this theorem as an independent interest question, and ask if there are PTAS for the same.
%\begin{theorem}\label{thm:part2}
%	There is a $O(1)$-approximation algorithm to cardinality constrained max-min allocation problem on uniform speed machines.
%\end{theorem}
%It is natural at this point to ask the complexity of cardinality constrained max-min and min-max allocation problems on unrelated machines. For makespan minimization, Saha and Srinivasan~\cite{SS} in fact give a $2$-approximation which matches the best known algorithm without cardinality constraints. They do so by using the natural assignment LP relaxation augmented with cardinality constraints and describe a rounding algorithm.
%The max-min problem, however, is notoriously difficult~\cite{bibid} even without the cardinality constraints -- {\em describe results.} There are $O(1)$-algorithms known for the restricted-assignment max-min allocation problem~\cite{bibid} which we denote as $P|restr|C_{min}$ (also known as the Santa Claus problem); this is the same setting as $P||C_{min}$ except some jobs are disallowed on some machines.
%
%One can reduce the cardinality-constrained max-min allocation problem to the restricted assignment max-min allocation problem in the following straightforward manner. Given a guess $T$ for the optimum value, in the optimum solution machine $i$ must be allocated
%a subset of jobs $J$ such that $\sum_{j\in J} p_j \ge Ts_i/2$ {\em and} $p_j \geq Ts_i/2k_i$ for $j\in J$. Therefore, if we restrict jobs $j$ to machines $i$ only if $p_j \ge Ts_i/2k_i$, then solving this restricted assignment max-min allocation problem {\em without} cardinality constraints would give a $O(1)$-approximation. In short, the $O(1)$-approximation algorithms for the Santa Claus problem imply $O(1)$-approximation algorithms for $P|k_i|C_{min}$. Unfortunately, we do not know $O(1)$-approximation algorithms for $Q|restr|C_{min}$; all the $O(1)$-algorithms for restricted-assignment max-min problems go via classifying jobs as big or small (for all machines), and it is not clear whether the various $O(1)$-algorithms~\cite{BS, Feige, Ola, AFS}  for Santa Claus generalize to this case. We leave this as an interesting open question.
%

\subsection{Outline of Techniques} \label{sec:overview}
As mentioned before, we obtain our results by reducing \mckc~{\em to} the \cckp problem (complementing the {\em from} reduction  discussed in Remark~\ref{rem:cckp}).
We provide two reductions -- the first incurs logarithmic approximation to the cost but uses black-box algorithms for \cckp, the second incurs $O(1)$-approximation to the cost but uses ``LP-based'' algorithms for \cckp.
%Both these reductions proceed via {\em decomposing} the given \mckc instance. %\smallskip

\medskip \noindent {\bf Warm-up: Weak Decompostion.}
Given a \mckc instance, suppose we \emph{guess} the optimal objective value, which we can assume to be $1$ after scaling. Then, we construct a graph connecting client $j$ with facility location $i$ iff $d(i,j) \leq 1$.
Then, starting at an arbitrary client and using a simple region-growing technique (like those used for the graph cut problems~\cite{LeightonR99,GargVY96}), we can find a set of clients $J_1$ of along with their neighboring facility locations $T_1 = \Gamma(J_1)$\footnote{For $S \subseteq C \cup F$, $\Gamma(S)$ denotes the neighboring vertices  of $S$.}, such that: (a) the diameter of $J_1$ is $O(\log n/\epsilon)$, and (b) the additional clients in the boundary $|\Gamma(T_1) \setminus J_1|$ is at most $\epsilon |J_1|$. Now, we simply \emph{delete} these boundary clients and charge them to $J_1$, incurring a capacity violation of $(1+\epsilon)$. Moreover, note that in an optimal solution, \emph{all} the clients in $J_1$ \emph{must be} assigned to facilities opened in $T_1$. Using this fact, we define our first demand in the \cckp instance by $D_1 = |J_1|$ and $f_1 = |T_1|$. Repeating this process, we get a collection of $\{(J_i,T_i)\}$ which naturally defines our \cckp instance. It is then easy to show that an $\alpha$-approximation to this instance then implies an $(O(\log n/\epsilon),  \alpha(1+\epsilon))$-bicriteria algorithm for \mckc.

\iffalse
The weaker decomposition theorem (Theorem~\ref{thm:weakdecomp}) states that we can delete a subset $\Cd$ of clients and partition the residual instance into portions we call {\em complete neighborhood sets} (Definition~\ref{def:comp-nbr}) of $O(\log n/\epsilon)$ diameter.
These sets consists of subsets of facilities $T_i$ and clients $J_i$ such that the optimal solution \emph{must} assign clients in $J_i$ to facilities in $T_i$. This collection of complete-neighborhood sets then naturally leads to a \cckp instance (Remark~\ref{rem:red})
whose solutions translate to \mckc solutions with $O(\log n/\epsilon)$ hit on the cost. Furthermore, the deleted clients $\Cd$ can be charged to clients in $C\setminus \Cd$ such that the capacity of facilities only increase by an $\epsilon$-factor.
We use the {\em region growing technique} which have been used for cut problems~\cite{LeightonR99,GargVY96} to find the set $\Cd$; we keep on growing balls till the total external demand is at most $\epsilon$ times the internal demand.
$O(\log n/\eps)$-radius balls suffice. %\smallskip
\fi

\medskip \noindent {\bf LP-Based Strong Decompostion.} %It is not a-priori clear how to modify the above technique to obtain better factors for the distance objective.
To get $O(1)$-approximations, we resort to linear programming relaxations. Indeed, one can write the natural LP relaxation \eqref{eq:lp1}-\eqref{eq:lp6} described in Section~\ref{sec:prelims} -- the relaxation has $y_{ip}$ variables which denote opening a
facility with capacity $c_p$ at $i$.
Armed with a feasible solution to the LP, we prove a \emph{stronger decomposition theorem} (Theorem~\ref{thm:decomp}): we show that we can delete a set of clients $\Cd$ which can be charged to the remaining ones, and then partition the remaining clients and facilities into {\em two} classes.
One class $\calT$  is the so-called \emph{complete neighborhood sets} of the form $\{(J_i, T_i)\}$ with $\Gamma(J_i) \subseteq T_i$ as described above --- we define our \cckp instance using these sets. The other class $\calS$  is of, what we call, {\em roundable} sets (Definition~\ref{def:rnding-mkc}). Roundable sets have ``enough'' $y$-mass such that installing as many  capacities as prescribed by the LP (rounded down to the nearest integer) supports the total demand incident on the set (with a $(1+\epsilon)$-factor capacity violation). Moreover, the diameter of any of these sets constructed is $\tilde{O}(1/\epsilon)$.

\medskip \noindent {\bf Technical Roadblock.}
It may seem that the above decomposition theorem implies a reduction to the \cckp problem -- the class $\calT$ defines a \cckp instance and we can use black-box algorithms, while the roundable sets in $\calS$ are taken care of almost by definition. The nub of the problem lies in the {\em supply} of capacities to each of these classes.  Indeed, the \cckp instance formed from $\calT$ must have a solution if the \mckc problem is feasible, {\em but only if all the $k_p$ copies of capacity $c_p$ are available to it.} However, we have already used up some of these copies to take care of the $\calS$ sets, and what we actually have available for $\calT$ is what the {\em LP prescribes.} In fact, this natural LP relaxation (and the natural LP for \cckp) have arbitrarily bad integrality gaps, even for bicriteria algorithms.%, that is, although the LP is feasible, any assignment will violate capacities to $\Omega(n)$ factors.% \smallskip

\medskip \noindent {\bf The Supply Polyhedra.} We circumvent this issue in the following manner: the above method would be fine if the supply of facility capacities prescribed by the LP to the complete-neighborhood sets in $\calT$ can approximately satisfy the demands in the corresponding \cckp instance. This motivates us to define {\em supply polyhedra} for \cckp. Informally, the supply polyhedron (Definition~\ref{def:supp-poly}) of a \cckp instance is supposed to capture all the vectors $(s_1,\ldots,s_n)$ such that $s_j$ copies of capacity $c_j$ can approximately satisfy the demands of all the machines. Conversely, any vector in this polyhedron should also be a feasible (or approximately feasible) supply vector for this instance.

 If such an object $\calP$ existed, then we could strengthen our natural LP relaxation as follows. For {\em every} collection $\calT$ of complete-neighborhood sets, we add a constraint (described as \eqref{eq:lp7}) stating that the fractional capacity allocated to the facilities in $\calT$ should
 lie in the supply polyhedron of the corresponding \cckp instance. Note that this LP has exponentially many constraints, and it is not clear how to solve it. However, we can use the ``round-and-cut'' framework (of inferring a separating hyperplane if our rounding fails, and then using the ellipsoid algorithm overall) exploited earlier in many papers~\cite{CarrFLP00,ChakrabartyCKK11,AnSS14,DemirciL16,Li15,Li16}.
 %Starting with a solution $(x,y)$, we use the strong decomposition theorem to obtain the set $\calT$ and check if the restriction of $y$ to the facilities in $\calT$ lies in the supply polyhedron of the corresponding \cckp instance. If yes, then we are done.
 %If no, then we have obtained a separating hyperplance for the super-large LP\eqref{eq:lp1}-\eqref{eq:lp7}, and we can run the ellipsoid algorithm.
 Using this decomposition, in~\Cref{thm:reduction}, we effectively reduce \mckc to the task of designing good supply polyhedra for \cckp.

\medskip \noindent {\bf Supply Polyhedron for \cckp and $Q||C_{min}$.}
Do good supply polyhedra exist for \cckp or even the simpler $Q||C_{min} $ problem?
On the positive side, we show (Theorem~\ref{fthm:asslp}) that the natural assignment LP is a $2$-approximate supply polyhedron for $Q||C_{min}$. For \cckp we describe a supply polyhedron based on the {\em configuration LP} and prove that it is $O(\log D)$-approximate (Theorem~\ref{thm:conflp}) where $D$ is the ratio of maximum and minimum demand. This along with our strong decomposition proves Theorem~\ref{thm:2}. We note that this also implies a {\em polynomial time} $O(\log D)$-approximation algorithm for the \cckp problem, improving considerably over the guarantees implied by the current santa-claus algorithms. %Our algorithm (described in Section~\ref{sec:conflp}) proceeds by massaging a given LP solution till it yields.
%\comment{Do we want to add a line on how we get these results}
We complement this by showing (Theorem~\ref{fthm:conf-ig}) that the integrality gap of the configuration LP is $\Omega(\log D/\log\log D)$, using which we also show a \emph{lower-bound} on the approximation factor possible using supply polyhedra: any supply polyhedra for \cckp must violate the demands by $\Omega(\log D/\log \log D)$. This shows that our approach inherently needs to violate capacities by this factor.

%On the other hand, using fairly standard tricks of enumeration and rounding, we can provide a QPTAS for \cckp (Theorem~\ref{thm:q}). We leave the complexity of \cckp as an interesting open question.

%\paragraph{Supply Polyhedra.}




%We start by writing the natural assignment LP relaxation for the problem. As is usual, we guess $\opt$ and scale everything such that $\opt = 1$.
%We have opening  variables $y_{ip}$ for every $i\in F,p\in [P]$ indicating whether we open a facility with capacity $c_p$ at location $i$.
%We have connection variables $x_{ijp}$ indicating the fraction to which client $j\in C$ connects to a facility at location $i$ where a type $p$ facility has been opened.
%We force $x_{ijp} = 0$ for all $d(i,j) > 1$.
%If $\opt = 1$, there is a feasible $(x,y)$ solution to the following system of inequalities.\smallskip

%\begin{minipage}{0.45\textwidth}
%	\begin{alignat}{4}
%		& \quad \forall j\in C,   &&\quad  \textstyle \sum_{i\in F} \sum_{p\in [P]}  x_{ijp} \geq 1 \label{eq:lp1} \\
%		& \quad \forall i\in F,p\in [P] ,  &&\quad  \textstyle \sum_{j\in C}  x_{ijp} \leq c_py_{ip} \label{eq:lp2} \\
%		& \quad \forall p\in [P], && \quad \textstyle \sum_{q \geq p} y_{iq}   \leq \sum_{q\geq p} k_q \label{eq:lp3}
%	\end{alignat}
%\end{minipage}
%~\vline~
%\begin{minipage}{0.45\textwidth}
%	\begin{alignat}{4}
%		& \quad \forall i\in F, j\in C,p\in [P],  && \quad x_{ijp} \leq y_{ip}\label{eq:lp4}   \\
%		& \quad \forall i\in F, && \quad \textstyle\sum_{p\in [P]} y_{ip} \leq 1 \label{eq:lp5}  \\
%		& \quad \forall i\in F,j\in C,p\in [P], && \quad x_{ijp},y_{ip} \geq 0\label{eq:lp6}
%	\end{alignat}
%\end{minipage}
%\smallskip

%For technical reasons, we have written \eqref{eq:lp3} as a constraint on the prefix-sums rather than individual capacities. However, a feasible integral solution satisfying \eqref{eq:lp3} can easily be converted to a feasible solution satisfying individual capacities.

%\paragraph{Integrality Gap.}
%The above LP has bad integrality gap even when we allow arbitrary violation of capacities.
%Consider the following instance. The metric space $X$ is partitioned into $(F_1\cup C_1) \cup \cdots \cup (F_K\cup C_K)$, with $|F_k| = 2$ and $|C_k| = K$ for all $1\le k\le K$.
%The distance between any two points in $F_i\cup C_i$ is $1$ for all $i$, while all other distances are $\infty$. The capacities available are $k_1 = K$ facilities with capacity $c_1 = 1$ and
%$k_2= K-1$ facilities with capacity $c_2 = K$. It is easy to see that integrally any solution would violate capacities by a factor of $K/2$.
%%It is easy to see that the above instance is not feasible with $OPT=1$: indeed, there is at least one client location where the optimal solution does not place a facility of capacity $H$ in its neighborhood, and it is not possible to serve the demand of this client using only capacity $1$ facilities, as there are only two locations where we can place facilities in its neighborhood.
%On the other hand, there is a feasible solution for the above LP relaxation: for $F_k = \{a_k,b_k\}$, we set $y_{a_k2} = 1-1/K$ and $y_{b_k1} = 1$, and for all $j\in C_k$, we set $x_{a_kj2} = 1-1/K$ and $x_{b_kj1} = 1/K$.
%%
%%
%%fractionally assign $1-\frac1H$ units of capacity-$H$ facility and $1$ unit of capacity-$1$ facility in the neighborhood around each client. It is easy to see that there is a feasible fractional assignment of this kind which means that the LP suffers from an unbounded (w.r.t the guessed objective function value) integrality gap.
%
%
%\paragraph{Decomposition Theorem.}
%The integrality gap suggests we need to strengthen our LP, and we will indeed do so. However, the above LP suffices to tease out the instance into parts that are indeed ``well roundable'' and problematic parts which look like the example above.
%To make this precise, let us introduce two definitions.
%\begin{asparaitem}
%	\item A subset of facilities $S$ is said to be {\em $(a,b)$-roundable wrt a feasible solution $(x,y)$} to \eqref{eq:lp1}-\eqref{eq:lp6} if its diameter is at most $a$ and there is a rounding $Y_{ip}\in \{0,1\}$ for all $i\in S,p\in [P]$
%	such that the rounded solution satisfies cardinality constraints, and  has enough capacity to satisfy $1/b$th of  the {\em fractional} demand incident on $S$. In other words, if we install $b\cdot c_p$ capacity at the location where $Y_{ip} = 1$, then it can satisfy the fractional demand incident on $S$.
%	%That is, if we increase the capacities by $b$ times, there is an integral rounding of facilities in $S$.
%	\item
%	A subset $S$ of facilities is called a {\em complete neighborhood} if there exists some clients $J\subseteq C$ such that $S$ contains all the facilities in distance one to clients in $J$.  That is, for all $j\in J$, the only facilities $i$ with $x_{ijp} > 0$ must lie in $S$.
%	Note that in the integrality gap example above, the $F_k$'s are all complete neighborhoods due to the client set $C_k$'s. Also note that these complete neighborhood sets are also encountered in the reductions from $3$-Partition and the cardinality constrained scheduling problems.
%\end{asparaitem}
%
%Note that if our instance can be partitioned into roundable sets then we would be done. If our instance consists of only complete neighborhood sets, then we could hope to use techniques developed for scheduling algorithms. However, a priori, the instances are a mixture of both.
%Our main technical hammer is the decomposition theorem (Theorem~\ref{thm:decomp}) which says that given feasible solution $(x,y)$ to \eqref{eq:lp1}-\eqref{eq:lp6}, in polynomial time we can decompose the instance $(F\cup C,d)$ into two collections $\calS$ and $\calT$ where
%every set $S$ in $\calS$ is a $(\tilde{O}(1/\eps),(1+\eps))$-roundable set, and every set $T\in \calT$ is a complete neighborhood set of diameter $\leq 4$. This tells us that the core difficulty that the above LP faces are indeed complete neighborhood sets of small diameter, and shows us how to strengthen our LP relaxation. {\bf Maybe add a few lines on how we obtain -- connections to region growing algorithms.} \medskip
%
%\noindent
%Next we describe two ways to strengthen the LP. One leads to a polynomial time algorjthm but gives $O(1)$-factor violation of the capacities, the other leads to a quasipolynomial time $(1+\eps)$-factor violation in the capacities. Both LPs, put extra constraints on the vector
%of $y_{ip}$'s. Interestingly, both LPs have exponentially number of variables and constraints we do not know if either LP is polynomial or quasipolynomial time solvable. Rather, we use the ``round-and-cut'' strategy~\cite{bunch fof citations} where the constraints+auxiliary variables are added
%in phases {\em only if} a rounding algorithm fails. This technique has led to many new algorithms in the recent past, and ours adds to this canon of growing work.
%
%\paragraph{LP strengthening.} One useful idea that has helped for scheduling problems~\cite{bibid} is to look at {\em configuration LP}. For our problem, we add the following constraint. For a subset of clients $J\subseteq C$ let $\Gamma(J)\subseteq F$
%be the facilities at distance $1$. Since $J$ can only be assigned to clients in $\Gamma(J)$, there must be enough capacity installed on $\Gamma(J)$ -- in particular, the multiset/configuration  $S$ of capacities must be of cardinality $\le |\Gamma(J)|$ and total capacity $\geq |J|$.
%We strengthen our LP~\eqref{eq:lp1}-\eqref{eq:lp6} by adding that for every $J\subseteq C$, the $y_{ip}$ vector must {\em dominate} a feasible configuration LP solution for the complete neighborhood $(\Gamma(J),J)$.
%
%As mentioned above, this huge LP is perhaps not solvable in polynomial time. Instead we add these constraints iteratively. In every phase, given a feasible $(x,y)$ to \eqref{eq:lp1}-\eqref{eq:lp6}, we apply our decomposition theorem and obtain the complete neighborhood sets and add the strengthened constraints for these sets. The analysis of the ellipsoid algorithm implies in polynomially many phases we will reach a solution $(x,y)$ where the $y$'s satisfy the configuration LP constraints for all the complete neighborhood sets.
%Our final contribution is an $O(1)$-rounding of the configuration LP. {\bf deepc: maybe expand on this as well.}
%
%



\subsection{Related Work}\label{sec:related}
Capacitated Location problems have a rich literature although most of the work has focused on versions where each facility arrives with a predetermined capacity and the decision process is to whether open a facility or not.
We have already mentioned the state of the art for capacitated $k$-center problems.
For the capacitated facility location problem a $5$-approximation is known via local search~\cite{BansalGG12}, while more recently an $O(1)$-approximate {\em LP-based} algorithm was proposed~\cite{AnSS14}.
All these are true approximation algorithms in that they do not violate capacities. It is an outstanding open problem to obtain true approximations for the capacitated $k$-median problem.
The best known algorithm is  the recent work of  Demirci and Li~\cite{DemirciL16} who for any $\epsilon>0$ give a $\poly(1/\epsilon)$-approximate algorithm violating the capacities by $(1+\epsilon)$-factor.
The technique of this algorithm and its precursors~\cite{AnSS14,Li15,Li16}  are similar to ours in that they follow the round-and-cut strategy to exploit exponential sized linear programming relaxations.\smallskip

The \cckp problem is a cardinality constrained max-min allocation problem. There has been some work in the scheduling literature on cardinality-constrained min-max problem.
When all the machines are identical, the problem is called the $k_i$-partitioning problem~\cite{BabelKK98}.
When the number of machines is a constant, Woeginger~\cite{Woe05} gives a FPTAS for the problem, and the best known result is a $1.5$-approximation due to Kellerer and Kotov~\cite{KellererK11}.
To our knowledge, the related speeds case has not been looked at. When the machines are unrelated,  Saha and Srinivasan~\cite{SahaS10} showed a $2$-approximation; in fact this follows from the Shmoys-Tardos rounding of the assignment LP~\cite{ShmoysT93}.\smallskip

As we have discussed above, the \mckc problem behaves rather differently than the usual homogeneous capacitated $k$-center problem. This distinction in complexity when we have heterogeneity  in resource is a curious phenomenon which deserves more attention.
A previous work~\cite{ChakrabartyGK16} of the first two authors (with P.~Goyal) looked at the (uncapacitated) $k$-center problem where the heterogeneity was in the radius of the balls covering the metric space.
As in our work, even for that problem one needs to resort to bicriteria algorithms where the two criteria are cost and {\em number} of centers opened. That paper gives an $\left(O(1),O(1)\right)$-approximation algorithm.
In contrast, we do not wish to violate the number of capacities available at all (in fact, the problem is considerably easier if we are allowed to do so -- we do not expand on this any further).






